"I was Confused by It; It was Confused by Me:" Exploring the Experiences of People with Visual Impairments around Mobile Service Robots

Mobile service robots have become increasingly ubiquitous. However, these robots can pose potential accessibility issues and safety concerns to people with visual impairments (PVI). We sought to explore the challenges faced by PVI around mainstream mobile service robots and identify their needs. Seventeen PVI were interviewed about their experiences with three emerging robots: vacuum robots, delivery robots, and drones. We comprehensively investigated PVI's robot experiences by considering their different roles around robots -- direct users and bystanders. Our study highlighted participants' challenges and concerns about the accessibility, safety, and privacy issues around mobile service robots. We found that the lack of accessible feedback made it difficult for PVI to precisely control, locate, and track the status of the robots. Moreover, encountering mobile robots as bystanders confused and even scared the participants, presenting safety and privacy barriers. We further distilled design considerations for more accessible and safe robots for PVI.

==> Discussion/5-Discussion.tex <==
\section{Discussion}

Contribution.... We distill ...

\subsection{Accessible feedback modalities}
%BOTH BYSTANDER AND DIRECT USERS - mainstream robots in general
    1. Visual modifications
    2. Audible 
     Tactile cues --> 
        why better than audio - sound sensitive
        Limited functionality, used for control, cannot be used for tracking (specific position, exact location) but vibration for urgent info, attract attention

\subsection{Personal Robots vs shared robots} 
    
    Only for shared robots
    Authentication
    Psychological Security - tampering with items
    Multi-user ..  - Correct delivery (check if such delivery robots are there?), cannot see if there are multiple boxes for different deliveries -> wrong mental model; sanity concerns
    
\subsection{Direct user vs bystander}
    - differences between users and bystanders in terms of information needs
    only for Direct users - personal robots
    1. Fine control
    2. ACCESSIBLE INSTRUCTIONS
    
    - Safety and privacy concerns(lesser for direct users) between direct users and bystanders
    

    

\subsection{Disability-awareness robots}  
%If they were smart enough to tell you, or identify you and tell you something about themselves or what they were doing and proximity - bystanders (Thomas)

%Even for general users, ....

\subsection{Evaluation Metrics of Accessible Robots}

different layers of concerns - safety , privacy apart from accessibility -> cannot visually detect robot's presence or characteristics  -> so, not only consider accessibility but safety, privacy in BOTH perspectives -> unlike prior work that used only .. for evaluation -> but we  need to assess robot design based on safety ( and privacy); convey mental model of robot accessibly 


\prajna{Our research contributes the first thorough exploration of PVI's experiences with different types of mainstream mobile service robots. and sheds light on PVI's robot experiences as both users and bystanders. Through this research, we found} that robot users and bystanders have to mostly rely on visual feedback (visual displays, light indicators, etc.) while interacting with mainstream service robots since there is a lack of audible and tactile feedback on these robots. Consequently, these service robots become largely inaccessible for people with visual impairments, who then resort to alternative strategies, such as asking sighted companions’ assistance, to access the benefits of using these robots. The inaccessibility of the service robots’ features, for both robot users and bystanders, further gives rise to fear and anxiety regarding safety hazards and privacy violations posed by these robots. For example, while low-lying mobile robots pose as tripping hazards, aerial service robots pose the dangers of physical injuries and privacy violation. Moreover, PVI as bystanders also have a constant fear that flying service robots can encroach private property and invade bystanders’ privacy, which draws a parallel with prior research on drones with sighted bystanders \cite{butt2021deployment, LINTAN2021101462, vcaic2018service}. Possibly, increasing  awareness of the robot's features and functions using approaches accessible to PVI can help assuage most of the accessibility, safety and privacy concerns.

%%\subsection{Information needs for direct users and bystanders} 

%% To avert any form of privacy or safety hazard, service robot users and bystanders who have visual disabilities can be provided with accessible information regarding the robot’s location, status, and other features, as suggested by our participants. First, for all kinds of service robots, PVI, both users and bystanders, can be alerted about the location and proximity of the robots. In the case of drones, apart from its proximity, alerting about the drone’s altitude, speed, and purpose of flying can pacify the safety and privacy apprehensions of PVI bystanders with respect to flying drones. 

%%Additionally, providing information on the robot's status in an accessible form can ensure safe and comfortable PVI-robot interaction. For example, in the case of drones, having the ability to provide alerts to its user and nearby bystanders on the drone's failure due to damage can avert physical injuries due to crashes. Apart from aerial service robots, indicating the power status of domestic service robots to their users in an accessible way can help them understand if the robot needs to recharge and save the robot from getting its charge completely drained, thus preventing any form of tripping or physical injuries caused by accidentally bumping into a dead robot. Similarly, indicating visually impaired direct users if their robot requires maintenance can help them do the needful and maintain the robot’s lifetime. 

%%Further, service robots should provide accessible instructions on how PVI’s (both bystander and users) are expected to interact with them. For example, food delivery robots should provide accessible instructions to robot users on how to open the food compartment on the robot to pick up the food. For bystanders, the delivery robot should be able to alert its presence and either ask the bystander to move away or move away from the bystander by itself. 

%%\yuhang{Need a paragraph here as a transition paragraph. You can say something like, based on our findings from the study, we derive design guidelines (or considerations) to improve people's experiences with the mainstream robots, from direct user and bystanders' perspectives respectively. }

Based on our findings from the study, we derive design considerations to improve PVI's experiences with the mainstream robots, from direct user and bystanders' perspectives respectively.

\subsection{Accessibility enhancements for direct users} 
Based on our participants' experiences and suggestions, we derived four robot design improvement opportunities to enhance the robot accessibility and safety for visually impaired users.
    
    \textit{\textbf{Incorporating audible and tactile feedback.}} 
    %% REVISED %%
    %As depicted by our findings, PVI find it challenging to perform various functions of the robot, such as tracking the location and status of the robots, because of the lack of audio and tactile feedback from the robot. While participants started leveraging the existing audible feedback from the robot, such as the sound made by the robots, this audible feedback is not enough to perform the robot functions. Hence, the incorporation of audible and tactile feedback can be beneficial for PVI. 
    
    These types of feedback can be useful to PVI by twofold - first, improve accessibility of robot control and second, alert PVI about robot status, location, proximity, etc. in an accessible manner. %%In the first case, adding audible and tactile feedback could help PVI use the different modalities of robot control, such as buttons and joysticks. 
    In the latter case, perhaps, providing access to such types of information can not only enhance robot user experiences for PVI, but also help in preventing physical injuries, such as tripping over and accidentally bumping into robots. However, it should be noted that in the case of audible feedback, the sound level should be loud enough to be easily detectable but low enough to not bother people who are sensitive to sound.
    
    \textit{\textbf{Enhancing visual design for low vision.}} While people with low vision have the ability to use their limited vision to perceive robots with the help of visual indicators, as depicted by our findings, robot designers can make the visual cues on the robots more distinguishable. For example, the robot’s aesthetics can reflect high contrast to make them stand out amidst its surroundings.
    
    \textit{\textbf{Providing accessible instructions.}} \yuhang{Besides refining the robot design itself, providing accessible instructions on how to use a service robot is another important perspective that the designers and manufacturers should consider. In our study, we found that xxx}  For example, domestic service robot designers can provide audible robot set-up instructions, instead of written manuals. If the instructions are provided online, designers can make these instructions compatible with PVI’s assistive technology. In other words, robot designers can provide methods so that PVI’s can set-up their robots as easily as sighted people. In addition to instruction manuals, instructions provided by customer service agents can include more tactile cues and references to ensure effective communication between visually disabled users and sighted customer service agents.  

    \textit{\textbf{Intuitive fine grained control.}} Robot designers can develop ways of making specialized robot control intuitive for PVI. For example, drone designers can make the video stream obtained from the drone’s camera easily comprehended by users who are PVI, especially to avoid obstacles during navigation. Further, designers can also come up with ways for PVI to easily correlate between joystick movements/button presses and drone's movements.
    
\subsection{Accessibility enhancements for bystanders} 
Besides direct users, bystanders experiences with service robots can be also improved in terms of the accessibility of the service robots, as mentioned below.
    
    \textit{\textbf{Providing audible cues.}} In addition to visual indicators, audible cues can be helpful to alert the presence of a moving robot to people who are totally blind. These audible cues can be provided before approaching bystanders, so that they have sufficient time to react to an approaching robot. Further, these cues can take the form of simple beeping or verbal output from robots. In the latter case, robots can verbally announce the purpose of the robot and indicate its intended direction of movement via speech. In this way, PVI could navigate sidewalks without the anxiety of being in the presence of an unknown moving object. %If they were smart enough to tell you, or identify you and tell you something about themselves or what they were doing and proximity.
    
     \textit{\textbf{Inclusion of visual indicators.}} Particularly for mobile robots travelling in public spaces, visual indicators can alert bystanders with low vision about an approaching robot. These indicators can warn people with low vision about the mobile robot’s presence and help them take necessary actions to move away from it.
     
\subsection{Regulating the use of service robots in public with proper policy.} Besides recommendations for robot designers, lawmakers are also important stakeholders to ensure safe robot experiences for PVI in public. Lawmakers need to regulate proper use for public service robots. As John pointed out, there needs to be laws that limit people who can fly drones in public spaces to ones who have the necessary training to control it. This would ensure that drones fly safely and could prevent any dangerous situations like sudden drone crashes from occurring in public spaces without any warning. Hence, with the existence of safe drone control policies, especially bystanders with visual impairments, can feel comfortable in its presence. A similar rationale can be drawn for delivery robots, where policies regarding its use of sidewalks must be administered for pedestrians' safety. As stated by prior work \cite{bennett2021accessibility}, mobile robots can block sidewalks for pedestrians making it dangerous for them to navigate through sidewalks and cross traffic. This can be particularly difficult for PVI since they may not be able to detect the presence of these mobile robots on the sidewalks. Hence, laws that regulate the use of such mobile robots on public grounds must be enforced so that the compact sidewalks and other curbs meant for PVI are not blocked by these robots.
    
%% Where does this fall?
Another approach to improve the accessibility of mainstream robots for PVI, which can be beneficial for both bystanders and direct users, is preserving robot's power. Robot designers can include a mechanism for robots to maintain residual power, so that robots always have the ability to use its audible and visual indicators. 
    
\subsection{Human-Awareness Robots}
Despite having accessible cues, it could be possible for PVI to either not be able to comprehend the robot’s efforts of interaction or not be able to react in the expected manner because of their disabilities. Hence, as stated by Thomas, robot designers can provide mobile robots with the capability to recognize people with disabilities and take necessary actions to preclude potential confusion and danger. For example, mobile robots could identify people with disabilities and steer away from their paths to avoid hitting or tripping them over. 

\subsection{Limitations and Future Work}

While this research produces a variety of contributions in the field of service robots, the primary drawback of our study is that it was conducted with participants whose experiences with mainstream service robots were not uniformly distributed across the three mobile robots. To overcome this limitation in future, we will recruit equal number of participants for each robot type. Further, it was not possible to conduct contextual inquiry study with our participants because of COVID-19 restrictions.

%%% REVISED %%%
%While this research produces a variety of contributions in the field of service robot accessibility for PVI, there exists some scope for improvement. This study was conducted with participants whose experiences with mainstream service robots were not uniformly distributed across the three mobile robots. This was because we recruited participants who had experiences with at least one of the three mainstream service robots. For our future work, we could recruit equal number of participants for each robot type. However, this type of recruitment comes with a caveat that there are quite a few PVI who use delivery robots and drones compared to vacuum robots, as shown in \ref{fig:survey}. Hence, the number of participants in each category would be limited. 

%Apart from the non-uniform distribution, we could not conduct a contextual inquiry study to physically observe PVI's interactions with service robots. This was mainly due to the COVID-19 restrictions on conducting in-person studies.




    




==> Discussion/Copy_Discussion.tex <==
\section{Discussion}
%%context awareness technology
%%Direct use of service robots 
%%      How to enable fine-grained control by providing continuous feedback 
%%      Accessible instruction 
      
%%Bystander
%%      Inform needs
%%      Inform robot intent accessibly 
%%       Protect privacy accessibly 
%%       Policy

%%Shared robots
%%       Security 
%%       Confusion


Our research presents the first thorough exploration of PVI's experiences with different types of mobile service robots. Moreover, unlike most prior work that focused on the direct use of the robots \cite{gadiraju2021fascinating, forlizzi2006service}, our research paints a comprehensive picture of PVI's robot experiences by taking into account both the direct users' and bystanders' perspectives. Our study revealed PVI's concerns, needs, and expectations for mobile service robots. We found that the interfaces of mobile service robots lack enough audio and tactile feedback, posing severe barriers for PVI. As a result, PVI adopted different coping strategies (e.g., listening to the robot noise to distinguish the robot position), AI-based technologies, and human assistance (e.g., remote agent service) to support their interactions with the robots. Moreover, we found that mobile service robots were a source of fear and anxiety for PVI, especially when they were bystanders around the robots. Participants expressed concerns on tripping over a moving service robot and their privacy being violated by robots with sensors (e.g., camera).

Based on PVI's experiences and suggestions from our study, we derive design considerations to inform more accessible and safe mobile service robots for PVI. 

\subsection{Accessible Interaction with Robots as Direct Users }  
Inaccessible feedback and control were the major reasons that hindered effective interaction between PVI and the robots. Based on our finding, we discuss four directions to enhance PVI' interactions with service robots as direct users. %---enhancing robots' visual design for people with low vision, providing options for customizing robot feedback, improving accessibility of fine-grained robot control, and incorporating accessible instructions.
%visual feedback was the primary feedback modality used by mobile service robots, such as the visual displays on a robot controller, the indicator lights on a drone, and the visual map of a space generated by a vacuum robot, which made it challenging for PVI to understand the robot's status and location. Even for low vision participants who have residual vision, the current visual feedback was not always accessible. We discuss how to provide more accessible feedback for people with visual impairments, including both low vision and blindness.

\textbf{Incorporating alternative and customizable feedback.} Current robot interfaces mainly rely on visual feedback to communicate robot information to users. To make a robot universally accessible, audio and haptic feedback should be added as alternatives to fulfil the needs of users with diverse abilities. Moreover, our study showed that different visually impaired participants also have different preferences on feedback modalities. For example, while audio feedback is accessible for PVI and commonly used by our participants to infer the robot's status (e.g., the noise made by the robot), this feedback can be frustrating for PVI who are highly sensitive to sound (e.g., John). Hence, haptic feedback, such as vibrations and textures, can be more beneficial in this situation. With each type of feedback having its own pros and cons, robot designers should consider providing users more flexibility to customize the feedback based on their abilities and preferences. %For example, a sound-sensitive and visually impaired user could have the option to mute the sound made by the press of buttons on the robot. They could instead use the button textures to distinguish one button from another. 

\textbf{Enhancing visual design for low vision.} While audio and haptic feedback is needed for people with little to no vision, we found that participants with low vision (e.g., Ara, John) can still perceive the robots via different visual feedback, such as the contrast between the robot and its background, the indicator light, and the information on the visual display. However, most visual cues are not visible enough to low vision users due to the small size and low contrast against the background, preventing low vision people from leveraging their residual vision. Besides adding more feedback alternatives, robot designers should consider making the visual cues on the robots more distinguishable to benefit low vision users who prefer using their vision. For example, the robot’s appearance itself should reflect high contrast to avoid the effect of its background on the robot visibility. The light indicators should be bigger and brighter, and adopt different blinking patterns instead of colors to indicate different robot status, thus diminishing the barriers for people who are color blind.  

%and possess brighter indicators to make the robot and its indicators stand out amidst its surroundings.

\textbf{Enabling fine-grained control.} Fine-grained control of the robot, such as accurately controlling the movement of a robot without running into an obstacle, is one biggest challenge for PVI. While participants could leverage some existing but limited audio feedback (e.g., the robot noise) to infer basic robot information, such as whether the robot is nearby, such feedback was not informative and precise enough to support a precise control of the robot. Enabling accessible fine-grained control for PVI is challenging since it requires both accurate localization of the robot and real-time feedback to communicate such information. To address this problem, our participants suggested using AI-based technology or human agents to track and convey the robot's position and status, such as whether the robot is approaching an obstacle. In fact, prior research in HRI has investigated computer vision algorithms for robot tracking and collision detection. Moreover, Gadiraju et al. \cite{gadiraju2021fascinating} has also explored PVI's preferences on the input and output modalities when piloting a drone, although no systems have been implemented and evaluated. Future research should consider how to combine the state-of-the-art AI technology with suitable feedback to enable precise robot control for PVI. 

%From these observations, we identified two main points of discussion---first, what are the different ways of obtaining complex information (e.g., robot's location and its environment) for fine-grained control and second, how can this information be communicated accurately while being accessible to PVI. While various prior work has focused on computer vision to enhance real-time fine-grained robot control via multiple sensors (e.g., cameras) for sighted people \cite{schmidt2021real, patel2021event}, the main challenge for robot designers is developing solutions that are also accessible to PVI. As reported by recent prior work \cite{gadiraju2021fascinating}, fine-grained drone control can be enhanced by incorporating specialized audio tones (e.g., beeping while approaching obstacles) and haptic feedback (e.g., vibrations from wrist bands) to acquire complex information on the drone's environment. However, robot designers need to consider validating these suggestions for accessible use of mobile robots and weigh the considerations against other factors including PVI' sensitivity to sound. 


%Hence, robot designers should consider including distinguishable audio, or even verbal feedback, to alert PVI about 

\textbf{Providing accessible instructions.} Besides refining the robot design itself, providing accessible instructions on how to use a service robot is another important perspective that needs attention from the designers and manufacturers. Our study uncovered two major reasons cause the accessibility issues of the robot instructions. First, the instructions are presented in an inaccessible format, for example, many robots provided only printed manual books, which are difficult for PVI to perceive. Second, the instruction content itself is visual-oriented, using different visual cues to provide guidance. As mentioned in our study, even the human agents from the customer services rely on visual cues to describe the robot components to our visually impaired participants. To enable PVI to fully benefit from the robot, it is important for manufacturers o provide accessible usage instructions. For example, robot set-up instructions should have an alternative audio version. Additionally, customer services should provide training to enable agents to properly communicate with people with disabilities and provide suitable guidance. %instructions provided by customer service agents can include more tactile cues and references to ensure effective communication between visually disabled users and sighted customer service agents.

%%Inaccessible feedback was one major reason that hindered effective interaction between PVI and the robots. From our study, we found that visual feedback was the primary feedback modality used by mobile service robots, such as the visual displays on a robot controller, the indicator lights on a drone, and the visual map of a space generated by a vacuum robot, which made it challenging for PVI to understand the robot's status and location. Even for low vision participants who have residual vision, the current visual feedback was not always accessible. We discuss how to provide more accessible feedback for people with visual impairments, including both low vision and blindness.

    

\subsection{Space Sharing with Robots as Bystanders}
While all kinds of detailed information is needed from the robots to enable direct interaction, we found that when encountering mobile service robots as a bystander, PVI care more about how to protect themselves regarding both physical safety and privacy. We discuss PVI's needs around mobile robots as bystanders. 

%From our study, we identified two unique considerations to enhance HRI for PVI as bystanders---PVI' distinctive information requirements for safe and comfortable mobile robot experiences, and needs for policies on the use of service robots in public spaces.

%difference between direct users' and bystanders' experiences with mobile service robots---while PVI as direct users require multiple types of information and feedback from the robot to effectively interact with them  (e.g., robot's power status, task completion status, etc.), bystanders only need information that would help them feel safe around these robots. In other words, bystanders' perspectives of their interaction with mobile robots is mostly limited to understanding the purpose of use and direction of movement of the robot for their own navigation purposes. 

\textbf{Conveying Robots Intent.} Effectively communicating the robot intent to bystanders is an important topic in the human-robot interaction (HRI) field to ensure bystanders' safety. HRI researchers have designed different methods to visualize the robot's moving trajectories for sighted bystanders \cite{watanabe2015communicating, walker2018communicating}. However, our study showed that bystanders with visual impairments need more information to feel safe and comfortable around a mobile robot. We summarize the information requirements for bystanders with visual impairments: (1) existence of the robot: whether there is a robot nearby; (2) proximity: how far away the robot is; (3) movement status: whether the robot is moving and when it will move; (4) moving information: which direction is the robot currently moving in or intends to move, and at what speed the robot is moving. Unlike prior work that focused on visualizing the robot's intent, robot designers need to consider how to effectively convey this information to PVI in an accessible and unobtrusive manner. %For example, the robots could talk to help PVI understand what the robot is being used for, and in which direction the robot is moving, as suggested by Thomas. Moreover, designers should also consider using cues that do not distract PVI and disrupt their attention while navigating public spaces.

%While prior research has developed methods for robot intention communication for sighted bystanders , robot designers also need to consider conveying the five information types to PVI in accessible ways. 

\textbf{Communicating Privacy-related Information.} Bystanders face privacy risks since they lack the knowledge of the robot's design and capability. In our study, we found that such risks can become severe for bystanders with visual impairments since they cannot visually observe the robots to detect the sensors (e.g., cameras, microphones), thus estimating and avoiding the potential risks. %As expressed by our participants, PVI are apprehensive that service robots could have sensors, such as cameras and microphones, capable of capturing unsolicited information from bystanders. 
Participants indicated three key types of information about the robots that can help them better understand the robot and protect their privacy: (1) existence of sensors: whether sensors capable of capturing bystanders' information are present on the robot; (2) purpose of data collection: why the robot is being used and why specific information is collected; (3) data collection scope: what range of data the sensor is capturing (e.g., the field of view of the camera), and whether the visually impaired bystander is involved in the data collection. While various prior work in privacy has explored sighted bystanders' privacy perception and exceptions around robots, such as drones \cite{wang2016flying, yao2017privacy}, no research has deeply investigated the unique privacy perceptions and needs for bystanders with visual impairments. Researchers and designers in HRI and privacy should consider how to accessibly convey the sensor information on robots to foster privacy equity for bystanders with visual impairments. 

%Similar to methods for conveying robot's intent, robot designers could communicate the robot's sensorial information via verbal feedback from the robot. Robot designers could also develop accessible smartphone applications capable of detecting the various sensors present on the robot and conveying the relevant information to bystanders.   

\textbf{Policies to regulate robot behaviors.} Besides having the robot communicate different types of information to PVI to alleviate their safety and privacy concerns, laws and policies are also needed to ensure the proper use of mobile robots in public spaces. As shown in both our study and prior work \cite{bennett2021accessibility}, mobile service robots occupy sidewalks, parks, beaches, and other public spaces, creating navigation difficulties for people with disabilities. Some states in U.S. have passed laws that limit robot use in public spaces. For example, San Francisco law administered by Norman Yee restricts the number and speed of delivery robots that can travel on sidewalks at any given time. This law also requires delivery robots to have permits to operate in public and the presence of trained human operators at all times \cite{LawDelRobot}. However, not all states have laws restricting robot use in public. For example,  With the growth of the service robot market, the government should enforce responsible robot deployment and use in public via regulations to protect the right of bystanders with diverse abilities. For example, one of our participants John suggested a law that only people with proper certifications could fly a drone in public to reduce the dangerous situations caused by a drone crash. 

%Because of the absence of laws for robots' use, even the spaces meant for people with disabilities are blocked for use by these robots posing safety hazards to PVI \cite{bennett2021accessibility}

%Moreover, the occurrence of dangerous situations, such as drone crashes, could be decreased if law mandates robot users to undergo training on how to safely control robots in public. Hence, with the regulation of mobile robot control, people with diverse abilities and mobile service robots could share public spaces in harmony. For example, John pointed out that there needs to be laws that limit people who can fly drones in public spaces to ones who have the necessary training to control it. This would ensure that drones fly safely and could prevent any dangerous situations like sudden drone crashes from occurring in public spaces without any warning. 





%%While bystanders do not require complex information from the robots for effective HRI, they possess more safety and privacy concerns compared to direct users. This is mostly because PVI as bystanders lack the awareness of the moving robot's presence, intentions and characteristics, since they cannot perceive an approaching robot. As described by Thomas, PVI could get confused on how to react in a safe manner when approaching a mobile robot in public. To circumvent these apprehensions, robot designers need to consider ways to alert bystanders about an approaching mobile robot. To do this, the robots could have audio and visual indicators to indicate its proximity. The robots could also talk to help PVI understand what the robot is being used for and in which direction the robot is moving, as suggested by Thomas.  

%%Meanwhile, direct users also need to understand how to control and use the robot efficiently, as described in the following paragraphs.

   %% \textit{\textbf{Enhancing fine-grained robot control.}} First, as reported in our findings, PVI find it difficult to achieve fine control of robots, especially in the case of drones, since they cannot visually see the robot's movements and its surroundings. Hence, robot designers should consider developing ways of making fine-grained robot control more accessible for PVI. For example, drone designers can make the video stream obtained from the drone’s camera comprehensible for users who are PVI, especially to avoid obstacles during navigation. Further, designers can also come up with ways for PVI to easily correlate between joystick movements/button presses and drone's movements.
    
    %%\textit{\textbf{Improving accessibility of instructions.}} Besides refining robot control, providing accessible instructions on how to use a service robot is another important perspective that the designers and manufacturers should consider. In our study, we found that most robots come with written instruction manuals, which are inaccessible to PVI.  Thus, robot designers need to consider providing instructions that make PVI set-up their robots as easily as sighted people. For example, designers can consider providing audible robot set-up instructions, instead of the inaccessible written manuals.  In addition to instruction manuals, instructions provided by customer service agents should include more tactile cues and references to ensure effective communication between visually disabled users and sighted customer service agents. (delivery robot, confused about use?)

\subsection{Design Considerations for Shared Robots} 
Compared to personal robots that a user can fully control, our study showed that the professional robots shared by multiple users (e.g., delivery robots) posed unique challenges and concerns to PVI. We discuss the unique features of professional shared robots as well as design suggestions to make them more accessible.   

    \textbf{Ensuring secure robot sharing.} Security is one major concern when multiple people share one robot. Our visually impaired participants have also expressed security concerns when authenticating to the delivery robot service. To enable accessible authentication for PVI, prior research has explored the accessibility issues and security concerns faced by PVI when authenticating to websites and applications on computers and smartphones \cite{dosono2015m, hayes2017they}. Accessible authentication mechanisms, such as UniPass \cite{barbosa2016unipass}, have also been developed to help PVI securely and easily log into their computers and smartphones. However, it is unclear whether such authentication methods could be applied to robots directly. To ensure a secure robot sharing experience, future research should explore PVI's authentication needs in the context of shared robots, determining whether the existing accessible authentication mechanisms could be directly adapted to shared robots or new methods would be needed for accessible robot authentication. %no authentication  With the burgeoning use of service robots, designers need to consider if the conventional accessible authentication techniques can be adapted to shared robots as well or if secure and accessible techniques need to be developed for robots altogether. 
    
    %Our participants suggested having more accessible and secure ways to obtain robots' shared services.
    
    
    %%Unlike personal robot users, shared robot users need to authenticate to the service of the robots before using it. As conveyed by our findings, users with visual impairments can either be unaware of the existence of authentication methods (Ara) or be unsatisfied with the existing authentication approach, such as text-message based authentication (John). Thus, robot designers can look into incorporating more accessible and secure ways of authenticating to the service of robots, including assistive technology compatible multi-factor authentication. 
    
    %Change title from auth 
    %prior work on authentication for PVI, our research stressed that PVI actually care about auth,  can prior tech be adapted to robots? Will it be easy and accessible?
    
    \textbf{Avoiding confusion caused by shared use.} Beside security concerns, shared robots can also confuse users when it comes to picking up the right order amongst multiple orders. This is especially true for users with visual impairments, who cannot perceive the physical features of the robot. For example, a food delivery robot could have multiple food orders in its compartment(s) for multiple users. As reported by our participants, it can be confusing for users with visual impairments to deduce which order they are supposed to pick up from the robot. Hence, with robots expanding to serve multiple users at a time \cite{}, robot designers need to consider how robots can help PVI discern which service is meant for them, thus promoting orderly use of shared robots' services.
    
    %Another design consideration for shared robots is that robot designers could incorporate accessible methods to indicate PVI if they have availed the service that was meant for them. Once the service is complete, the robot could also indicate the completion to the users. This could be particularly helpful in situations where the robot handles multiple services at a time. Alerting PVI in accessible ways could avoid confusion about picking the right service from the robot.  
    
    %Another concern reflected by our findings on the delivery robots' use is that it can be confusing for shared robot users with visual impairments (e.g., Ara) to understand if they have availed the service from the robot that was meant for them. in the case of a single robot handling multiple deliveries, robot designers should consider ways of indicating PVI which is the right order and confirming the delivery completion.
    
    %For example, though Ara's robot delivered only one order at a time, she feared if she had picked up the right order. 
    %There are two implications that can be drawn from Ara's concerns. First, PVI can derive the wrong mental model about service robots, which can create confusion and anxiety. Thus, robot designers should consider giving robots the capability to provide accessible information to PVI about the features and functions of the robots. 
    %Second, in the case of a single robot handling multiple deliveries, robot designers should consider ways of indicating PVI which is the right order and confirming the delivery completion. 
    
    %Remove mental model
    

\subsection{Context-aware robots}

In our study, participants suggested that service robots should intelligently understand PVI' abilities, situations, and needs to enhance their interactions with the robots. One of the reasons favouring context-aware robots is that PVI may not identify cues from the robots. For example, as reported by Ara, the robot's audio feedback may be dampened by the environmental noises making it difficult for PVI to understand the robot's location. Consequently, PVI may not react in ways to effectively interact with the robots and avoid dangerous situations. Hence, as stated by Thomas, robot designers could provide mobile robots with the capability to recognize people with disabilities and take necessary actions to preclude potential confusion and danger. For example, mobile robots could identify people with disabilities and steer away from their paths to avoid hitting or tripping them over.

In addition to disability awareness, robot designers could also make service robots perceive PVI' status. For example, as reported by our participants, the vacuum robots continuously emit feedback even if the users are not at home. Eventually, the robot's power gets exhausted leaving the users confused about the whereabouts of the robot when they return home. As a solution to this problem, robot designers could include the feature where the robot identifies the absence of users (users' status) and does not send out audio feedback to alert its status, thus preserving its power to emit feedback when the user returns. 




%%\subsection{Evaluation Metrics of Robots}

%%Conventional roboticists have primarily focused on evaluation metrics related to the generic usability and technology of the robots, such as robot failure frequency, system usability, (humna-robot trust) etc. \cite{}. However, even the commonyly used rop=obots are not accessible to PVI. Hence accessibility should be considered. safety, pshych security, privayc, of sighted people. involve people with dicverser abilities. This research sheds light on the various dimensions of robot design including accessibility, safety, and privacy for both robot users and bystanders. As reported by our findings, mobile service robot design is not accessible to 


%While prior work has mostly focused on technology-related accessibility guidelines for robot users, such as ensuring "perceivable displays" and "operable hardware controls" \cite{qbilat2021proposal}, this research sheds light on the various dimensions of accessible robot design including safety and privacy for both robot users and bystanders. Since PVI do not have the ability to clearly perceive the presence and characteristics of mobile robots, it is not surprising that they get anxious about their safety and privacy in the presence of these robots. Hence, robot designers should consider gauging the safety and privacy of PVI in the presence of the mobile service robots in addition to evaluating the accessibility of the technology itself to determine if the robot can potentially become mainstream for everyone, including PVI as users and bystanders. 
    
%How do robot designers evaluate accessibility of robots? Did they consider safety and privacy?
%How can robot designers evaluate safety and privacy of robots?

==> Findings/4-Findings.tex <==
\section{Findings}

\subsection{General Use of Mainstream Robots}
Participants have various experiences with the three types of mobile service robots as direct users or bystanders. All participants own or have used a vacuum robot, two have used the delivery robot service at most four times, and five have experiences of controlling a drone. Besides directly using the robots, participants have also encountered robots that are not owned by them. Three participants have come across a vacuum robot at a friend’s place, four have encountered delivery robots on the sidewalk (two of them mentioned that they ran into delivery robots frequently), and seven participants have come across drones in public spaces such as parks and beaches. Moreover, two participants reported that they had used other types of robots, including a robot mop (Tim) and autonomous driving vehicles (Thomas), as shown in Table 1. 

The frequency of use of the vacuum robot ranged from daily (5/17 participants) to "seldom use during the pandemic" (1/17 participant). All the vacuum robots were at least one year old, and was used to clean the entire house/apartment. Four out of the five participants used a drone only once, while only one participant used it twice. Two participants used the drone inside their houses and three used the drone in parks.  



%when they got vacuum robot
%when they used delivery robot
%when they got a drone

%where do you use the robot - vacuum robot, drones

%how frequently do you use vacuum robot/drone/delivery service

\subsection{Motivation of Using Robots}

%Participants used service robots for different reasons. Similar to sighted people \cite{forlizzi2006service},

Participants used service robots for different reasons. Similar to sighted people \cite{forlizzi2006service}, most participants use a vacuum robot because it allows them to multitask, thus saving their time. However, three participants (Jen, John, and Meg) use vacuum robots because of their disabilities. They indicated that the vacuum robot enabled them to complete the cleaning task that they cannot easily accomplish on their own. As John said, “I have physical disabilities that prevent me from doing a lot of moving around. Also just, you know, being able to see the dirt and stuff is difficult, so having the robot take care of that was the idea behind buying it.”

The two participants who used the delivery robot mentioned that they used the service because it is convenient, efficient, and cheaper compared to the food delivery services by humans. Ara mentioned, “You know, I could just order what I wanted and then have the robot come and bring it to me. So, it definitely was time saving and convenient.” Moreover, John emphasized the potential low cost of robot delivery and how the robot can save human efforts, especially in challenging situations:

\emph {“Well, I like that I didn't have to tip the robot. It is nice not to have to pay any extra or feel sorry for this person having to come out in the rain today so I'm going to tip them extra, because you don't feel sorry for the robot having to go out in the rain to get the food.”}

In terms of the drone, most participants (5 out of 6) purchased it for their children as a toy and have only played with it occasionally by flying it around. Only one participant, Samuel, bought a drone for himself to reach inaccessible places of this house. Samuel has low vision and could leverage his functional vision to control the drone using a joystick and use it to reach high places that he cannot access. He described how he used the drone to inspect and solve an issue on the roof of his house:

\emph{“We have places that are, you know, many meters up above ground level that you could only reach with an extremely long ladder and I do not like ladders. We have had problems with wasp nests in the roof and I thought about for a long time how to deal with that without climbing a ladder. And I came up with this idea that if I had a good drone, I could actually attach something like a, you know, a length of very lightweight stiff wire and then maybe like a ball soaked in insecticide and I can fly [the drone] out there [to drop the insecticide].”}

\subsection{Interacting with Robots as Direct Users: Accessibility Issues, Strategies, and Needs}

While benefiting from the mainstream robots, participants also face various challenges and concerns during their interaction with the robots. We report participants’ interaction experiences, challenges, and strategies when using the three types of robots, respectively, based on the main tasks associated with each robot.

\subsubsection{Vacuum Robots}
While facing some accessibility challenges, all participants are able to use the vacuum robots to clean their houses. The interaction with vacuum robots includes two major tasks: controlling the robot (e.g., start or stop the robot), and tracking the robot's location and status.

\textbf{(1) Controlling the robot} 

Participants reported three approaches to control the vacuum robots, including directly pressing the physical buttons on the robot, remotely controlling the robot via a mobile application, and using speech commands via a smart speaker.
    
\textit{\textbf{Physical buttons on the robot.}} All the vacuum robots used by the participants have at least one control button, such as the start button, located on their surface. Thirteen participants used these buttons to manually control the robot. However, most participants (12 out of 13) had difficulty distinguishing the physical buttons on their robots since the buttons were all flat and blended into the robot surface. Only Ahmed felt that the control buttons were accessible since the start button on his robot had a tactile feature, which made it easy to recognize. However, most robots do not provide such tactile buttons. 

\begin{figure}[h]
  \centering
  \begin{subfigure}{.5\linewidth}
    \centering
    \includegraphics[width=0.5\linewidth]{Sections/tactile_button.png}
    \caption{Tactile Start Button}
    \label{fig:sub1}
  \end{subfigure}%
  \begin{subfigure}{.5\linewidth}
  \centering
  \includegraphics[width=0.5\linewidth]{Sections/nontactile_button.png}
  \caption{Non-tactile Start Button}
  \label{fig:sub1}
\end{subfigure}%
\caption{Tactility of the start button on vacuum robots}
\end{figure}
            
To use the physical buttons, participants have to memorize each button’s location and its function, which increases their cognitive load. As Ara mentioned, “It's very difficult to kind of place [the buttons] and [map] what button is what, and remember that.” Some participants also leverage AI-based assistive technology. For example, Rita used the Seeing AI application to recognize the functionalities of the non-tactile buttons on the vacuum robot. Participants suggested multiple ways to make the buttons more distinguishable, such as presenting the buttons in different shapes or textures (John and Rita), or adding tactile symbols or braille to label the button functions (e.g., Ahmed, Thomas). 
            
 \textit{\textbf{Manufacturer's smartphone application.}} Some vacuum robots come with a smartphone app for users to interact with the robots (e.g., the iRobot HOME App for Roomba). Six participants use the manufacture smartphone application to control their robots. They all appreciate the fact that the application supports a variety of functions including scheduling a cleaning task, locating the robot when stuck, and showing the robot status to the user. However, these applications are not always accessible. While visually impaired people can use a screen reader\footnote{Screen readers are software programs that identify the elements displayed on a screen and repeat that information back to the user, via text–to–speech or braille output devices \cite{screenReader}. When using a screen reader on a smartphone, a user can conduct specific gestures to set focus on a user interface component and receives audio description of that component. Typical screen readers on smartphone include VoiceOver for iOS and TalkBack for Android.} to access smartphone applications, the applications for vacuum robot do not work well with the screen readers. Many components on the application user interface are not labeled with accessible text needed by a screen reader. As Rita described, “The controls to navigate through the time selections [for scheduling a cleaning task] weren't very accessible... It wasn't clear which selection [button] did what...” While having a screen reader on her phone, she expressed that the virtual buttons in the application were “as elusive as” the physical buttons on the robot. Participants' difficulty with the vacuum robot's phone application has echoed the long-standing button accessibility problem in smartphone applications \cite{ross2018examining}. 
            
Besides the basic buttons, some vacuum robot applications have an advanced mapping feature---the robot scans the whole space to generate a visual map, and the user can then use this map to divide their house into different sections, name the sections, and assign specific sections to the robot to clean. Seven participants mentioned this feature to us. While the participants believed that this feature could be potentially useful since they could ask the robot to clean specific rooms without vacuuming the whole house, labeling different rooms on the visual map is extremely challenging for them to accomplish. Tim described his experience with the map feature:

\textit{"That whole marking and labeling of the individual rooms is not accessible. It's a visual map that shows up on the [phone] screen and you have to distinguish one room from another and once you have those rooms kind of laid out, then you can go through and label them as kitchen, living room, whatever. Because that is inherently a visual process working with the map, I've never been able to do it.”}


As an alternative to the visual map, Tim suggested assigning the target cleaning area to the robot in a more intuitive manner, such as assigning the target area via the user's location, "Because the map feature wasn't really accessible, I would like to be able to tell the robot to follow me. And then when I got to my room or wherever and I wanted to start cleaning, I could just say start, start cleaning.”

            
\textit{\textbf{Speech Commands via Smart Speaker.}} Besides the above control methods that come along with the robot, five participants also connected their vacuum robots to a smart speaker, such as Alexa and the Google Home speaker, so that they can control the robot with speech commands. As Edward said, "I tell Alexa to send [the vacuum robot] home, and it would go back to the docking station.” Apart from basic controls such as start and stop the robots, Cathy also used Alexa’s services to understand the location of the robot: “You can ask [Alexa] to locate [the vacuum robot], and [the robot] will start making a sound of where she is.”
            
While limited control functions are supported by the smart speaker compared to the phone application, two participants preferred using a smart speaker since it is more efficient and supports hands-free interaction with the robot. As Edward mentioned, “I overall prefer to use Alexa. Once it was set up, I found it to be faster than pulling out my phone and going into the app and looking for the button that I wanted.”

However, two participants (Edward and Sara) struggled with connecting the smart speaker to the vacuum robot. As a result, they have to turn back to the smartphone application or the physical buttons. 
            
\textbf{(2) Tracking robot location and status}

Tracking the robot is another important task when using vacuum robots, especially for visually impaired people who may accidentally trip over moving robots. Besides location, vacuum robot, being a complex system, also requires users to track its status from multiple aspects, such as the power status, the status of the dirt bin level, and whether the robot is stuck. Participants can use different indicators from the robot to understand its status, including haptic, audio, and visual notifications. The following paragraphs report the various approaches used by participants to understand the whereabouts and status of the robot and the challenges they face. 
        
\textbf{\textit{Tracking by sound.}} One major strategy that all participants use to track the robot's location and status is listening to the noise made by the robot as it vacuums. The disappearance of noise indicates that the robot is either stuck or has completed its cleaning task. If the robot is not present in its docking station, the participants deduce that the robot is stuck. To help users locate the stuck robot, some advanced robots can generate a beeping sound to inform the user. Eleven of our participants mentioned that they use the smartphone application or the smart speaker to make the robot beep when they want to find the robot. 
            
The worst situation is when the robot runs out of power while getting stuck. The robot is thus not able to generate any noise or audio indicator, which makes it extremely hard for the visually impaired participants to find it.  All the participants expressed their concerns regarding this situation.
            
\emph{“Sometimes it will go dead while it's stuck [when I'm not at home], because every few minutes, the robot gives another notification, and that runs down its battery, so I wish there was a way for me to tell it like ‘I know you're stuck but I can't do anything right now [since I’m not at home]” (Reena)}
            
To locate an out-of-power robot, participants have to physically get down and scan the whole room. Thomas described his efforts to manually find the robot by using his cane: “When [the robot] wasn’t running, I didn't know where it had stopped, you know, I had to get down on the floor with my cane and swipe around until I found it, and it was tucked away under some table when it stopped by itself.” 
            
To ease the process of locating a dead robot, some participants (Rita, Tim) memorized the places where the robot usually gets stuck. They either search these areas first when they lose track of the robot, or prevent the robot from getting into these problematic areas in the first place by blocking its way with obstacles. Further, all the participants expressed that the robot should be able to save some amount of power instead of continuously notifying the status and getting the charge completely drained. The residual power could then be used by the user to locate the robot using the robot's audio indicator. Moreover, Tim also suggested that the smartphone application for the robot should store the latest position of the robot, so that the users can easily locate the robot even when it is out of power. 
            
Although the noise and audio feedback could be helpful for visually impaired people, participants who are sensitive to noise (John and Reena) found the robot difficult to use. For example, John has a hearing disability, which makes the robot cleaning noise painful for him to hear. He thus only starts the vacuum robot when he is out of home. However, the pandemic makes the situation more difficult since he cannot go out much. John described his experience:

\emph {“I use [the vacuum robot] seldom now since I don’t get out of the house in the pandemic. The vacuum is too loud for me to tolerate it being on in the house, which I know sounds a little crazy since I’m legally deaf, but I’m legally deaf because I score less than 40\% on word recognition and speech discrimination score. I’m actually hyper sensitive to both light and sound, so I cannot tolerate much light or sound. Unfortunately, pretty much all the robotic vacuums I’ve tried are just way too loud for me to coexist with in the house. So if I cannot leave the house, [I cannot use the robot].”}


\textbf{\textit{Tracking by visual information.}} Some low vision participants, who have residual vision, can visually locate the robot by observing the visual information on and around the robot, such as the contrast between the robot and the background, the light indicators, and other visual notification provided by the robot or its controller. 

\textit{Color Contrast.} Some low vision participants can see the robot if it has high contrast against the floor. As Ara mentioned, “I'm able to see the light and dark color contrast, and luckily the vacuums weren't the same color as the floor.” However, when there is no high contrast between the robot and the floor, it is difficult for the low vision participants to find the robot: “I wouldn’t be able to see where [the vacuum robot] was because it’s not contrasting with the carpet, because the carpet is dark as well. So, I had to like fumble around and try to find it, hoping I didn't step on it” (Ara).

Since it is hard to dynamically adjust the robot color based on the floor, participants suggested that the robot’s appearance itself should present a high contrast to be more visible. As Ara suggested, “If it were like a black vacuum, it could have like a white ring on the outside, or, you know, vice versa. So at least the thing has some contrast, and I'd be able to see it.”

\textit{Information on the robot display.} Some modern robots have a display to show its information to the users, such as the power status. Some low vision participants can read the information with the their residual vision and some vision enhancement tools. “[The robot] has a very large display on top that has a dark background with the light letters. I can actually read those if I magnify them with my iPad” (John). 
            
Unfortunately, for participants who are completely blind, the display feature was not accessible at all. Sara, who is totally blind, spoke about the inaccessibility of the display on the robot: “There's a display screen [on the robot] and I [am supposed to use] to go into the menus, but they are not accessible [because I'm totally blind].”
            
\textit{Light indicators.} Eight participants reported the presence of indicator lights on the robot, which would either blink or light up in different colours to indicate the status of the robot. Some low vision participants can use the light to locate the robot especially when the vacuum noise generated by the robot is dampened by other sound in the environment. As Ara said, "Like my fridge is going on and off, you know that can impede on the sound [of the vacuum robot], so then I have the light [to locate the robot]". 

 However, the light is not visible to all low vision participants due to its small size and low luminance. As John described, “There's an [light] indicator for how full the bin is, which is totally useless for me because I can't detect it. It's a tiny, tiny, little indicator.” Even for the low vision participants who can see the light indicators, it is difficult to understand the meaning of the lights. For example, while Ara's vision is good enough to see the lights, she is color-blind and thus cannot distinguish the color to figure out the implication of the lights. 
 
While some low vision participants can benefit from the light, it is completely inaccessible to people who are blind. For example, Jen described that the robot reset light was the only way to indicate whether the reset of the robot was successful. However, she cannot see the light, which makes it difficult for her to configure the robot. Instead of relying on visual cues, Jen emphasized the importance of having audible alternatives for the status alerts, "Because, you know, if you're blind, you're not going to be able to see the lights and know what's going on, so I think it's important for [the robots] to be as verbal and as interactive as possible."

\textbf{\textit{Tracking via Haptic Feedback.}} Apart from using audio and visual cues, one participant, John, also uses haptic feedback to track the robot status. His robot comes with a specialized remote controller (i.e., the FullCommand Remote for bObSweep PetHair Plus). When the robot gets stuck, the controller vibrates continuously to alert him. In general, John preferred haptic feedback the most compared to audio and visual feedback since it is a more universally accessible feedback that can be perceived by everyone, including people with multiple types of disabilities like hearing and visual disabilities. As he indicated, "For somebody like me [who is legally blind and deaf], the auditory and visual stuff, either is not useful or, you know, it might actually even be painful for me, but having the sense of touch is a universal identifier that everybody can associate with."

\subsubsection{Delivery Robots}
While xx participants have experiences with delivery robots, only two (John and Ara) have used a delivery robot service to get food delivered to their houses. Ara used the Starship robot, while John used Tech One Quick Serve. According to their experiences, four main tasks were associated with the delivery robot: locating the robot, authenticating to open the food compartment on the robot, picking up the right delivery, and dismissing the robot.

\textbf{\textit{Locating the robot.}} Once the food delivery order is placed, the first task is to locate the robot. John received text messages to notify him of the delivery arrival, while Ara used a website to track the robot location. However, the website relies on GPS and cannot locate the robot accurately in the last few meters. While sighted people can visually locate a nearby delivery robot, this last-few-meters way-finding problem is challenging for our participants with visual impairments\cite{saha2019closing}. Ara mentioned that she had to physically search for the robot when it arrived. 

\emph{“So I would check on the computer, because we have like a portal that you can log into to see where the robot was and where your food was, [but] it wasn't very specific. It was like, you know, say, your food is approaching your building. That's great, but when this building has several entrances, where's this thing going to meet me? So, I ended up like going outside of the building, walking around,and waiting for this thing to show up.”}

Besides locating the robots, physically reaching the robots can also be difficult. John raised his concern that the delivery robot cannot climb stairs, so he had to go outside his apartment building to find the robot. He emphasized this concern by explaining how navigating stairs could be difficult for people with visual impairments: “Stairs and blindness don't mix very well. So, it'll be nice if [the delivery robots] could get around the whole stair issue like the ability to deliver it in the apartment and not outside the building.” 

\textbf{\textit{Authenticating to the robot.}} John and Ara had different authentication experiences after locating the delivery robot. John authenticated to the delivery robot using text messages. %After successful authentication, he pressed a button on the robot to open the food compartment. %%Moreover, the authentication would fail if the user is not at the delivery location. 
%John mentioned that he could locate the button since its colour (red) contrasted with the colour of the robot (black). However, he felt that a person without colour perception could find it difficult to locate the button since it was "only half the size of his palm" and was "more or less flushed into the device". 
%%However, this authentication mechanism poses two problems. First, the food compartment button was difficult to locate on the robot; and second, if someone had access to his phone and was near the delivery location, the food could be picked up by the wrong person. Hence, he suggested enabling multi factor authentication or using an accessible mobile application to grant food compartment access to the user. 

On the other hand, Ara reported that there was no authentication required to pick up her delivery. She expressed her security concerns: "This [delivery robot service] didn't have any delivery authentication. This  thing [delivery robot] just showed up, and you would hope that it was your food.” She suggested that the delivery robot should incorporate more secure authentication mechanisms to ensure that the right person received the delivery. Further, John, who had to use text messages to authenticate his delivery, emphasized on the need for a more secure approach, such as, multi-factor authentication. 
    
\textbf{\textit{Picking up the delivery.}} Both John and Ara faced challenges when picking up the delivery from the delivery robots. Ara found it difficult to locate the food compartment on the robot, and she had to feel around the whole robot to find it. Since she has residual vision, she suggested adding some visual guidance to help her identify the food compartment, such as an arrow shaped light pointing to the food compartment. Meanwhile, John needed to press a button on the robot to open the food compartment. While he could locate the button because it since its color (red) contrasted with the colour of the robot (black), he emphasized that a person without color perception could find it difficult to locate the button since it was "only half the size of his palm" and was "more or less flushed with the rest of the device". 

Moreover, picking up the delivery from a low-lying robot could be difficult for people with motor disabilities. For example, besides visual and hearing impairments, John also experiences motor disabilities. It is difficult for him to bend down to pick up his food from the delivery robot. He thus suggested increasing the robot's height.

\textbf{\textit{Dismissing the robot.}} When the delivery task is completed, the lack of feedback on delivery completion confuses the participants. John reported, “[the robot] just moved away, I don't know, if I was totally blind, I might still be wondering, is [the delivery robot] just like sitting somewhere on my property or did it actually leave all the way.” Ara suggested that the robot should generate an audio notification once it was ready to leave. 
    
\subsubsection{Drones}
Six participants in our study have used drones. They reported three major tasks associated with drones: controlling the drone, obstacle detection during drone control, and tracking the location and status of the drone, as described in the following paragraphs.

\textbf{\textit{Controlling the drone.}} Participants reported two approaches to control the direction and speed of drones: joystick and buttons. However, both approaches are hard for the visually impaired participants to accurately control the drone movement. Without the ability of visually observing the drone's movements, the participants cannot understand the correlation between the joystick's movements and drone's actual behaviors. As Rita explained, “We couldn't tell how far to the left or to the right [the drone moved]. We couldn't measure, for example, if we wanted to go out 10 degrees to the right, we couldn't measure that with the joystick.” 

Some participants used buttons to control the drone movement, where the position of the button represents the moving direction of the drone (e.g., the drone moves to the left when pressing the left button). However, similar to the joystick, mapping the duration of button press with the movement of the drone was not an easy task to visually impaired users. As Rita described, "It's difficult to know how far it was going up with each press of the button and what happened when you didn't press a button. Was it staying hovering or was it kind of going down."

Moreover, using an additional controller can also conflict with the use of other assistive tools, such as a white cane. For example, John who uses a support cane reported that it was challenging for him to control a drone with a physical controller while holding his support cane. 

As a result, some participants suggest adding a speech input as a control alternative. For example, Samuel explained his struggle with the joystick and how speech control can reduce the learning curve：

\textit{"You have to sort of train with this these joysticks to get to where you feel like, Okay, I'm in control, there's training involved, it's not simple, I thought it would be really trivial to run this and then I started hitting walls... It's easier for me to say what I wanted to do than for me to remember that I gotta push this joystick at that angle... which is why I think it'd be nice if I could just talk to it and say now go over there you know now go left, go right, go up."}


\textbf{\textit{Obstacle avoidance.}} In addition to simply controlling the drone's moving direction, another important task is ensuring that the drone does not crash into obstacles. However, achieving this task is particularly difficult for people with visual impairments since they cannot visually detect obstacles in the path of the drone. For example, Samuel mentioned that his drone crashes many times because he cannot visually detect obstacles. Some participants (e.g., Ara, Rita) thus suggested providing audio description about the drone's surroundings via its camera or having an autopilot option for autonomous navigation. “It would either need to be able to tell me accessibly what it sees so I could fly it or it would have to have some sort of autopilot” (Ara).
    
\textbf{\textit{Tracking the drone location.}} Tracking the drone location is another difficulty faced by the visually impaired participants. While the drone usually has a camera that can stream its surrounding back to the user to help them track the drone, this feature is inaccessible to people with visual impairments. Instead, they could only estimate the drone's location based on the noise made by it propeller. As Rita said, "My husband and I are both totally blind. So you know, there is no audible output at all, so the camera was useless to us. The only way we knew where the drone was is because obviously it made a whirring sound."

However, the sound was not sufficient to inform the proximity and speed of the drone. Additionally, the drone sound annoyed some participants. For example, Thomas got nervous when hearing the noise since he felt that the drone was near enough if he could hear it. As he indicated, “[Drones] all make me very nervous. I don't like the sound, and I don't like the fact that I can't tell where they are. I don't like buzzing things flying around me.” 

Participants preferred receiving more audio feedback about the drone's location. For example, Rita suggested sending the camera's video stream to human service to get audio guidance. As she suggested, 

\textit{“I think the only other option we would have to make the drone accessible would be to connect your camera with some [human] assistance that would be able to give you verbal feedback…just to know where it is, the beeping [when approaching an obstacle] is enough but to get more details, then speech would be great. Or even if you had the option to talk directly to it and say, where are you, or what's your problem, and get some verbal feedback”}

\textbf{\textit{Tracking the drone status.}} Participants struggled understanding the drone's status, such as whether it's being charged and whether it encounters any problem. For example, Meg mentioned that the drone charging status was shown using an indicator light, which she could not see. Moreover, participants complained about that the drone did not have any form of audible feedback to alert if something was wrong with it.


    
\subsection{Safety Around Robots}
Besides the accessibility issues when directly using the robots, participants have emphasized the safety concerns around mobile service robots as direct users and as bystanders. While all three types of robots have posed safety risks to our visually impaired participants, participants perceived drones to be the most dangerous type of robots. Figure \ref{fig:safety} shows participants' mean perceived safety scores for different types of robots (perceived safety of vacuum robot: $mean = 5.94, SD = 0.82$; delivery robot: $mean = 5.40, SD = 3.05$; drone: $mean = 4.44, SD = 2.18$). We report participants safety perceptions around different robots from both direct users' and bystanders' perspectives. 

\begin{figure}[h]
    \label{fig:safety}
  \centering
  \includegraphics[width=0.75\linewidth]{Sections/safety.png}
  \caption{Average Safety Ratings (Scale: 1-7) for the Mainstream Robots. Note that the number of participants for each robot type is not the same.}
\end{figure}

\textbf{\textit{Safety concerns as direct users.}} Fifteen out of 17 participants consider the vacuum robot as a potential tripping hazard when it is in the middle of the room. Eight participants even expressed fear of tripping over their vacuum robots, especially when the robot runs out of power and stops (or gets stuck) at some places before getting back to the charging dock. Although no participant tripped over the robot, two participants (Tim and Meg) accidentally kicked the robot a few times, and one (Raya) almost tripped over it. Raya described her "near-tripping" experience:

\emph{"There are times when I don't know where [the robot] is and i think i can trip over it... There was one time when [the dead vacuum robot] was just kind of in the middle of the floor and, I almost tripped over it, but I caught myself in time.”}

Moreover, Samuel who had tunnel vision, expressed his frustration of visually watching out for the robot to avoid tripping: “Because I have low vision... one of my biggest headaches, is tripping over things unless I'm looking down. I have to be looking down specifically and around the house [to avoid tripping over the vacuum robot].” 

%%Surprisingly, no participants mentioned safety concerns when using delivery robots or drones.
Surprisingly, participants barely expressed safety concerns when using the delivery robots or drones as a direct user. Nina was the only one who felt unsafe when operating a drone because she was scared that it could hit her. 


\textbf{\textit{Safety concerns as bystanders.}} Besides the direct user experiences, encountering mobile robots as bystanders can also raise safety concerns. We focus on participants' bystander experiences with delivery robots and drones since participants rarely have bystander experience with the domestic vacuum robots. 

Participants felt confused and anxious when they run into a delivery robot on the sidewalk. They perceive the robot as an unfamiliar moving obstacle that has unclear intend and can potentially trip them. Thomas described his first encounter with a delivery robot:

\emph{"I encountered a robotic delivery device on the sidewalk in downtown San Francisco, and I was confused by it. And I think it was confused by me. I heard something on the sidewalk between loud traffic noises. And then, my cane detected [the delivery robot] and it was moving. And I think it stopped because my cane touched it. I reached out to see what my cane had touched that had been moving. And there was a box about the size of the shoe stand polishing box so it was probably 15 inches high by about 12 inches wide and 18 inches long, and I don't know what it was because I was by myself, but it moved. And I realized it was a box and it was probably a delivery box and when I got away from it, it started moving again and went on down the street. I was anxious about having heard it, having touched it with my cane and having it available to trip me."}

Moreover, Ara did not feel comfortable sharing the sidewalk with the delivery robots since they take over the limited navigation space that is already challenging for people with visual impairments, which aligns with the findings of Bennett et al.'s work \cite{bennett2021accessibility}. As Ara said, 

\textit{“The sidewalks are narrow and really don't have enough space to have a robot running around with other pedestrians and then you have yourself and people who have a guide dog, cane or whatever it may be, trying to navigate the sidewalk plus listening to these, you know, ambient sounds around you... so yeah, there's definitely a lot of hazards that come with [the delivery robot].”}

Interestingly, instead of worrying about the robot hurting themselves, some participants were concerned about their white cane getting broken by the delivery robot. As described by Jen, “I really didn't have any trepidation about [the delivery robot] hurting me physically or injuring me, but I definitely had concerns that it would definitely break my mobility [cane] and then I would have a bigger problem.”

Compared to delivery robots, participants expressed more safety concerns towards drones. Since it is an object flying at heights above humans, participants felt scared that the drone could fall and hit them when losing signal or power. Tina mentioned that since these drones could be flying at higher speeds, the reaction time to these incidents would be minimal. The situation could be more dangerous for people with visual impairments because they cannot see the drone to determine the necessary action to avoid danger. John elaborated on the potential danger of a drone: “You know, a blind person is not going to know when they need to put up their hands on their face defensively...if you don't know what it is like, you don't even know if it has any sharp thing or something on it, and you don't know whether it's propellers are moving, its propellers could cut me.” 

He commented that there should be a law that restricts drone controllers to people who have completed the specific training to fly these robots in a safe manner, ensuring that the drone does not hurt any bystanders.

\subsection{Privacy Concerns Around Robots}
Participants also expressed privacy and security concerns around the robots. When using vacuum robots, John, expressed his privacy concerns about it collecting xxx?. He mentioned that he did not like the use of GPS enabled applications since he felt unsafe to be tracked through the application. He further expressed his concerns on the unauthorized access to private data that smart devices with speakers and microphones can have: “Some people don't like using things like Alexa, because they, you know, are worried about their privacy, because of the devices having cloud access to data across the network that somebody else could be accessing and it's especially distressing if you're blind, that, you know, somebody else is watching you when you can't be watching them. A lot of times speakers make people uncomfortable because, you know, well, they have a microphone and, you know, it's listening to me, and stuff like that…”.

Moreover, six participants mentioned that their privacy could be violated as bystanders of robots, especially the drones since these drones could have the ability to trespass their private property or take pictures. They felt the drone "invasive and threatening" (Thomas). Samuel described his anxiety about being around drones: “There is an invasive quality, because it probably has a camera... It's almost like these people are watching us with their drones.” Moreover, the privacy risk could be more severe to people with visual impairments since they lack the ability to visually detect the drone and determine whether they are being captured. As Thomas said, “I don't want it coming over and inspecting me or hovering above my head...Also, where and why are big, big issues for me. Why is this thing here? What's it looking at? Am I involved? Is this observing me?”


\subsection{Sighted Assistance to Support Interactions with Robots}
To overcome the accessibility and safety issues posed by the robots, participants seek help from sighted people, including both acquaintances and remote agents. Twelve participants mentioned using human assistance when interacting with or encountering robots. 

\textbf{\textit{Help from sighted companions.}} Similar to prior research [cite], most participants (xx) asked their friends and family members to assist them when interacting with the robots. For example, when using the vacuum robots, participants asked their friends and family to help start the vacuum robot (xx), connect the robot to the robot application via WiFi or Bluetooth (xx), and identify the button functionalities (xx), and check the cleanliness of the floor after the vacuum robot finishes cleaning (Thomas).   

Moreover, when encountering robots on the street, participants sometimes rely on their sighted companions to help identify and avoid the robots. For example, Kat asked one of the sighted people around to tell her what the moving object was. Participants also felt safer with their sighted companions when encountering a robot. For example, Thomas felt less anxious when he was with his sighted friend compared to encountering the drone alone. As he indicated, “Fortunately, I was with my sighted walking partner, so I didn't get anxious about it, but if I was out here by myself I would be really worried because it sounds like it's close.” 

\textbf{\textit{Remote Agents.}} Seven participants used remote agent service via smartphone or smartglass applications (e.g., Be My Eyes \cite{bemyeyes} and Aira \cite{aira}) to conduct visual tasks, such as locating a stuck vacuum robot, and recognizing the non-tactile buttons on the robot. For example, Tim described his use of the mobile application, "Be My Eyes": “I use [Be My Eyes] like if I go to the usual spots where [the vacuum robot] is not there and I don't feel like crawling around on my hands and knees or whatever.”
    
\textbf{\textit{Customer Service.}} To use his vacuum robot, Tim always seeks help from the customer service. However, the instructions provided by a sighted agent is not helpful for him - The sighted agent uses only visual cues (e.g., colors of the robot components) as references during communication rather than tactile cues, which is not accessible to people with visual impairments. Tim described his experience where the customer service was giving him instructions to replace the brushes for his vacuum robots:
    
\emph{“There was a little bit of issues where they just couldn't communicate with me because, you know, they're sighted and I'm blind and the landmarks that they are using and trying to describe aren’t useful to me. So, you know, trying to get them to describe something to me in the language that I could understand, what I'm feeling versus what they're seeing...was a little bit of a challenge. For example, when you're going to replace the brushes underneath the [vacuum] robot. There's this tiny little lever that you have to squeeze this little trigger kind of thing in order to be able to open [the robot] and get the brushes. I couldn't get them to describe that tiny little lever because it's so small that if you don't know exactly what you're feeling for and where it is... It's pretty invisible, so I needed them to be able to say, okay, the lever that you're looking for is right next to this particular wheel right, next to this landmark or whatever, but they just kept saying, Oh, it's the blue lever... That doesn't do me any good. I need you to tell me, you know, is it near the left wheel or the right wheel, and depending on which way the robot is facing, you know, which way is left and which way is right.”}

Moreover, Tim expressed his disappointment about the customer service would not take his suggestions on improving the accessibility of the robot because of copyright infringement: 

\emph{“There's a large, large component of the technology built into this that I can't use. And the fact that, you know, when I call them and say hey, here's the problem that I have and here's, you know, as a blind person, a couple of easy solutions that I think would fix it, and they won't, and they refuse to listen to me, claiming that it could be a patent infringement if I give them an idea, and they run with it and build it into the robot, they're claiming I could turn around and sue them for copyright infringement.”}



==> Findings/4-Findings_NEW.tex <==
\section{Findings}

%% %% %% %% %%
\subsection{Mainstream Robots - Types of Experiences and Usage Patterns}

Participants have various experiences with the three types of mobile service robots as direct users or bystanders. All participants own or have used a vacuum robot, two (John and Ara) have used the delivery robot service at most four times, and six have experiences of controlling a drone. Besides directly using the robots, participants have also encountered robots that are not owned by them. Three participants (Meg, Nina, and Reena) have come across a vacuum robot at a friend’s place, six have encountered delivery robots on the sidewalks (four of them mentioned that they run into delivery robots frequently), and nine participants have come across drones in public spaces such as parks and beaches. Moreover, two participants reported that they have used other types of robots, including a robot mop (Tim) and autonomous driving vehicles (Thomas), as shown in Table  \ref{tab:demo}.

Participants who directly used the robots were further asked questions related to their usage patterns, including use frequency, area of use, and year of purchase/use, wherever applicable. The frequency of use of the vacuum robots ranged from daily use (5/17 participants) to "seldom use during the pandemic" (1/17 participant). All the vacuum robots were at least one year old, and were used to clean the entire house/apartment/workspace. Five out of the six participants who had experiences controlling a drone used it only once, while only one participant used it twice. Two participants (Meg and Samuel) used the drone inside their houses, three (Nina, Ahmed, and Rita) used the drone in parks and one participant (Reena) used her toy drone inside and outside her house. In the case of delivery robots, John used the service four times in the past one year and Ara used the service “since two years on and off”. 
%% %% %% %% %%





%% %% %% %% %%
\subsection{Motivation of Using Robots}

Participants use service robots for different reasons. Some of the motivations to use service robots were similar to the ones stated by sighted people in the existing literature \cite{forlizzi2006service}, \cite{iocchi2012domestic}. To begin with, participants (Ara and John) have adopted the use of robots because they find them convenient (Jen) and time-saving. As Ara expressed her intentions of using the delivery robot service -  “You know, I could just order what I wanted and then have the [delivery] robot come and bring it to me. So, it definitely was time saving and convenient.” In the case of domestic service robots like the vacuum robot, five participants (Samuel, Ahmed, Kat, Ara, and Rita)  feel they can multitask as the robot performs the household chores. 

In addition to the reasons that align with prior work with sighted subjects, our participants, who have visual impairments, use service robots to perform tasks that they cannot accomplish on their own because of their disabilities. John has motor disabilities in addition to visual disabilities. He feels that service robots help him accomplish his daily tasks without having to strain himself - “I have physical disabilities that prevent me from doing a lot of moving around. Also just, you know, being able to see the dirt and stuff is difficult, so having the [vacuum] robot take care of that was the idea behind buying it.”. Participants also reported the possibility of using robots to access places that are out of their reach. For example, Samuel bought a drone for himself to reach inaccessible places in his house. Samuel has low vision and could leverage his functional vision to control the drone using a joystick and use it to reach high places that he cannot access. He described how he used the drone to inspect and solve an issue on the roof of his house: 

\emph {“We have places that are, you know, many meters up above ground level that you could only reach with an extremely long ladder and I do not like ladders. We have had problems with wasp nests in the roof and I thought about for a long time how to deal with that without climbing a ladder. And I came up with this idea that if I had a good drone, I could actually attach something like a, you know, a length of very lightweight stiff wire and then maybe like a ball soaked in insecticide and I can fly [the drone] out there [to drop the insecticide].”} 

Besides using robots because of physical disabilities and to be able to reach inaccessible places, one participant, John mentioned an interesting point about the cost-effectiveness of using delivery robots:

\emph {“Well, I like that I didn't have to tip the robot. It is nice not to have to pay any extra or feel sorry for this person having to come out in the rain today so I'm going to tip them extra, because you don't feel sorry for the robot having to go out in the rain to get the food.”} 
%% %% %% %% %%





%% %% %% %% %%
\subsection{Interacting with Robots as Direct Users: Accessibility Issues, Strategies, and Needs}

While benefiting from the mainstream robots, participants also face various challenges and concerns during their interactions with the robots. Based on the interviews, we identified two primary tasks associated with the three mainstream robots -- controlling the robot and tracking robot's location and status -- and report participants’ interaction experiences, challenges faced, and strategies adopted when using the mainstream robots for each task. Additionally, we discuss participants’ experiences performing tasks that are unique to delivery robots and drones, respectively.

\textbf{(1) Controlling the robot} 

    Participants reported three approaches to control the robots, including directly pressing the physical buttons on the robot, remotely controlling the robot via a mobile application or a remote controlled device, and using speech commands via a smart speaker.

    \textit{\textbf{Physical buttons on the robot.}} Most of the robots that participants use have at least one button on its surface though the functionalities of the buttons vary from one robot to another. Our participants who had visual disabilities expressed that they can locate the buttons on the robot if the buttons have some form of tactile indicator, such as tactile symbols on the button, different button shapes, etc. However, most of the robots that the participants use have indistinguishable, non-tactile buttons. 

    All the vacuum robots used by the participants have at least one control button, such as the start button, located on their surface. Thirteen participants used these buttons to manually control the robot. However, most participants (12 out of 13) had difficulty distinguishing the physical buttons on their robots since the buttons were all flat and blended into the robot surface. Only Ahmed felt that the control buttons were accessible since the start button on his robot had a tactile feature, which made it easy to recognize. However, most robots do not provide such tactile buttons, as shown in Figure \ref {fig:sub2}.

    \begin{figure}[h]
      \centering
      \begin{subfigure}{.5\textwidth}
        \centering
        \includegraphics[width=0.6\linewidth]{Sections/tactile_button_cropped.png}
        \caption{}
        \label{fig:sub1}
      \end{subfigure}%
      \begin{subfigure}{.5\textwidth}
      \centering
      \includegraphics[width=0.6\linewidth]{Sections/nontactile_button_cropped.png}
      \caption{}
      \label{fig:sub2}
    \end{subfigure}%
    \caption{Tactility of the start button on vacuum robots: a) Tactile buttons; b) Non-tactile buttons}
    \end{figure}

    To use the physical buttons on the robots, participants have to memorize each button’s location and its function, which increases their cognitive load. As Ara mentioned for the vacuum robot, “It's very difficult to kind of place [the buttons] and [map] what button is what, and remember that.” Hence, participants suggested multiple ways to make the buttons on the robot more distinguishable, such as presenting the buttons in different shapes or textures (John and Rita), or adding tactile symbols or braille to label the button functions (e.g., Ahmed, Thomas). 
    
    Besides the non-tactility of the buttons on the robots, a unique problem was identified by the participants in the case of drones. Participants reported using two approaches to control its direction and speed: joystick and buttons. However, both approaches are hard for the visually impaired participants to accurately control the drone movement. Without the ability to visually observe the drone's movements, the participants cannot understand the correlation between the joystick's movements/duration of button presses and the drone's actual behaviors. As Rita explained, “We couldn't tell how far to the left or to the right [the drone moved]. We couldn't measure, for example, if we wanted to go out 10 degrees to the right, we couldn't measure that with the joystick.” 

    \textit{\textbf{Remote robot control via manufacturer’s smartphone application and remote controlled device.}} Some of the robots come with a smartphone application for users to interact with the robots (e.g., the iRobot HOME App for Roomba vacuum robot). They all appreciate the fact that the application supports a variety of functions associated with the robot, however, these applications are not always accessible. While visually impaired people can use a screen reader \footnote{Screen readers are software programs that identify the elements displayed on a screen and repeat that information back to the user, via text–to–speech or braille output devices \cite{screenReader}. When using a screen reader on a smartphone, a user can conduct specific gestures to set focus on a user interface component and receive audio description of that component. Typical screen readers on smartphones include VoiceOver for iOS and TalkBack for Android.} to access smartphone applications, the applications for the robots do not work well with the screen readers. In other words, many components on the application user interface are not labeled with accessible text needed by a screen reader. Participants' difficulty with the manufacturer's phone application echoes the long-standing button accessibility problem in smartphone applications \cite{ross2018examining}. 

    Six participants use the manufacturer’s smartphone application to control their vacuum robots. With the help of this application, participants can perform a variety of tasks including scheduling a cleaning task, locating the robot when stuck, and showing the robot status to the user. However, Rose and Rita reported that the application is not fully accessible to perform all these tasks. As Rita described, “The controls to navigate through the time selections [for scheduling a cleaning task] weren't very accessible... It wasn't clear which selection [button] did what...” While having a screen reader on her phone, she expressed that the virtual buttons in the application were “as elusive as” the physical buttons on the robot. 
    
    Besides the basic buttons, some vacuum robot applications have an advanced mapping feature---the robot scans the whole space to generate a visual map, and the user can then use this map to divide their house into different sections, name the sections, and assign specific sections to the robot to clean. Seven participants mentioned this feature to us. While the participants believed that this feature could potentially be useful since they could ask the robot to clean specific rooms without vacuuming the whole house, labeling different rooms on the visual map is extremely challenging for them to accomplish. Tim described his experience with the map feature:
    
    \textit{"That whole marking and labeling of the individual rooms is not accessible. It's a visual map that shows up on the [phone] screen and you have to distinguish one room from another and once you have those rooms kind of laid out, then you can go through and label them as kitchen, living room, whatever. Because that is inherently a visual process working with the map, I've never been able to do it.”}
    
    As an alternative to the visual map, Edward suggested assigning the target cleaning area to the robot in a more intuitive manner, such as assigning the target area via the user's location, "Because the map feature wasn't really accessible, I would like to be able to tell the robot to follow me. And then when I got to my room or wherever and I wanted to start cleaning, I could just say start, start cleaning.”
    
    In addition to the inaccessible mapping feature, Reena and Jen mentioned that their vacuum robot application notifies if something is wrong with the robot in the form of error numbers. However, these error numbers are not descriptive enough to understand what exactly is wrong with the robot. As Reena reported, "[The smartphone application] tells you an error number, how do you associate the error number to what the error is exactly. I have to hope it might be, say like, error 600: Roomba stopped, then I know what it was, but if it just says, sometimes it just says a number, and I don't know what it is." Hence, Jen suggested receiving more verbal description on what the error is in addition to the number.
    
    In addition to the inaccessible features of the vacuum robot application, two participants (Samuel and Sara) expressed their frustration with connecting the application with the robot, as Samuel described - “[The vacuum robot instructions] says go to your Android and download [the vacuum robot] app, it's free and put this app on your phone, and now your phone can talk to the robot. I did all that and they never communicated very well. [...] I uninstalled it and I reinstalled it and I played with it for a day and I just, I got impatient with it and said, All right, I don't need to talk to my robot on the phone.”
    
    In the case of drones, two participants (Samuel and Nina) mentioned using a smartphone application to control the drone’s movements. Similar to the vacuum robot phone application, Nina reported that the application was not accessible to her because of the incompatibility of the screen reader with the application. 
    
    Apart from the manufacturer’s smartphone application, seven participants (John, Summer, etc.) reported the use of a remote controlled device to control their robots. For example, Samuel, who had tunnel vision, described the vacuum robot’s remote controlled device as an accessible approach to control the robot - “there's [...] a little base that you put on the floor and plug into the AC, that’s it's charger and then you can just leave the remote there. So, every time I run [the vacuum robot], I just go, pick the remote up, and push one of the buttons [on the remote] and then it's, you know, then it [starts] [...] [The buttons on the remote controlled device are] easily accessible.” Furthermore, Rita, Ahmed, Meg and Reena used a remote controller to navigate their drones. Rita and Ahmed also had a display on their devices, which showed the drone camera's video stream. As Rita described, “[...] so the remote control was supposed to be able to work within a two mile distance to deliver [an object] and then come back. You should be able to fly it back [while looking] on the [controller’s] screen”. However, as mentioned previously, controlling drones with the joystick/buttons on the remote controller is not an accessible task for our PVI participants. More on the inaccessibility of the drone's camera stream will be discussed under the second mainstream robot task.
        
        
    \textit{\textbf{Speech Commands via Smart Speaker.}} This type of control is exclusive to vacuum robots, and is not observed in the case of delivery robots and drones. Besides the above control methods that come along with vacuum robots, six participants (Ahmed, Edward, Summer, Reena, Meg, and Jen)  also connected their robots to a smart speaker, such as Alexa and the Google Home speaker, so that they can control the robot with speech commands. As Edward said, "I tell Alexa to send [the vacuum robot] home, and it would go back to the docking station.” However, since the vacuum robot’s mapping feature is inaccessible to PVI, participants cannot ask the robot to clean specific areas of their houses using a smart speaker. More about the use of smart speakers will be discussed under the next mainstream robot task. 


\textbf{(2) Tracking robot's location and status} 

Tracking the robots’ location is another important task of robot interaction, especially for people with visual impairments who can accidentally bump into or trip over moving robots. Besides location, the system complexity of robots necessitates users to track its status from multiple aspects, such as tracking the robots’ power status, determining if the robot is stuck, etc. Participants can use different indicators from the robot to understand its status, including haptic, audio, and visual notifications. The following paragraphs report the various approaches used by participants to understand the whereabouts and status of robots and the challenges they face.

    \textit{\textbf{Tracking by sound.}} One major strategy that all participants use to track the robots’ location and status is listening to the sound made by the robots, especially while using vacuum robots and drones. The disappearance of the sound indicates that the robot is not in operation because it is stuck, has lost all its power, or has completed its task. Particularly in situations where the robot is incapable of generating any sound because of accidental crashes or loss of power in between operation, it becomes very difficult for participants to understand the location and status of the robot, thus creating anxiety and curiosity about the robot’s whereabouts. Hence, it is important to incorporate measures to ensure that robot users, who are PVI, are at least provided with the last known robot's location using accessible techniques, such as using a screen-reader compatible manufacturer's smartphone application, before such events occur.

    In the case of vacuum robots, the absence of noise indicates that the robot is either stuck or has completed its cleaning task. If the robot is not present in its docking station, the participants deduce that the robot is stuck. To help users locate the stuck robot, some advanced robots can generate a beeping sound to inform the user. Eleven of our participants mentioned that they use the smartphone application or the smart speaker to make the robot beep when they want to find the robot. However, the worst situation is when the robot runs out of power while getting stuck. The robot is thus not able to generate any notification, which makes it extremely hard for the visually impaired participants to find it.  All the participants expressed their concerns regarding this situation.  
    
    \emph{“Sometimes it will go dead while it's stuck [when I'm not at home], because every few minutes, the robot gives another notification, and that runs down its battery, so I wish there was a way for me to tell it like ‘I know you're stuck but I can't do anything right now [since I’m not at home]” (Reena)}
                
    To locate an out-of-power vacuum robot, participants have to physically get down and scan the whole room. Thomas described his efforts to manually find his vacuum robot by using his cane: “When [the robot] wasn’t running, I didn't know where it had stopped, you know, I had to get down on the floor with my cane and swipe around until I found it, and it was tucked away under some table when it stopped by itself.”  To ease the process of locating a dead vacuum robot, some participants (Rita, Tim) memorized the places where the robot usually gets stuck. They either search these areas first when they lose track of the robot, or prevent the robot from getting into these problematic areas in the first place by blocking its way with obstacles. Further, all the participants expressed that the robot should be able to save some amount of power instead of continuously notifying the status and getting the charge completely drained. The residual power could then be used by the user to locate the robot using the robot's audio indicator. Moreover, Tim also suggested that the smartphone application for the robot should store the latest position of the robot, so that the users can easily locate the robot even when it is out of power. 
                
    Although the noise and audio feedback can be helpful for visually impaired people, participants who are sensitive to noise (John and Reena) cannot tolerate the sound made by the robots and thus find the robots difficult to use. For example, John has a hearing disability, which makes the vacuum robot’s cleaning noise painful for him to hear. He thus only starts the vacuum robot when he is out of home. However, the pandemic makes the situation more difficult since he cannot go out much. John described his experience:
    
    \emph {“I use [the vacuum robot] seldom now since I don’t get out of the house in the pandemic. The vacuum is too loud for me to tolerate it being on in the house, which I know sounds a little crazy since I’m legally deaf, but I’m legally deaf because I score less than 40\% on word recognition and speech discrimination score. I’m actually hyper sensitive to both light and sound, so I cannot tolerate much light or sound. Unfortunately, pretty much all the robotic vacuums I’ve tried are just way too loud for me to coexist with in the house. So if I cannot leave the house, [I cannot use the robot].”}
    
    With respect to drones, one participant (Meg) mentioned that the sound made by them is not sufficient to understand the direction of the drone's movement. Meg reported that she cannot hear her drone well enough to control it smoothly without crashing it - “It wasn't really loud enough for me to navigate it without crashing easily.” The sound made by the drone was also not sufficient for participants to judge the drone’s proximity and speed. For example, Rita said - “The only way we knew where the drone was was because obviously it made a whirring sound. And that really didn't tell us how far it was, that didn't tell us anything.” Besides the sound level, participants also complained that the drone did not have any form of audible feedback to alert if something was wrong with it. While some participants preferred to receive more audio feedback from drones to discern its status and location, like in the case of vacuum robots, some participants (Thomas and Samuel) were annoyed by the sound made by drones. For example, Thomas got nervous when hearing the noise since he felt that the drone was near enough if he could hear it. As he indicated, “[Drones] all make me very nervous. I don't like the sound, and I don't like the fact that I can't tell where they are. I don't like buzzing things flying around me.” 
    
    
     \textit{\textbf{Tracking by smart speakers.}} In the case of vacuum robots, apart from basic controls such as starting and stopping the robots, participants (Meg, Reena, Edward, and Summer) used smart speakers to understand the robot’s location and status. For example, Edward used Alexa’s services to understand the status of the robot: “I would sometimes get an alert from Alexa [...] saying that [my vacuum robot] was stuck. [...]. [Otherwise, the status notification] was anything from, you know, your Roomba is charging or Roomba is 60\% charged or cleaning or docked, you know, [Alexa] gives different status messages like that.” Moreover, while the vacuum robot is powered, Reena can use her Echo Dot to determine the location of her vacuum robot: “[I use] Alexa to locate the Roomba, and that will make [the vacuum robot] make a sound, so I can go find it, but then sometimes [the vacuum robot] dies, and it doesn't go back to its charger, and then it takes me a really long time to find where it went.”  

    Not all participants preferred to use a smart speaker with their vacuum robots since not all smart speakers provided robot status alerts in addition to robot control. For example, Jen reported that the functionality of her smart speaker was limited to asking Alexa to clean specific areas of her house. However, with the inaccessibility of the mapping feature, as specified under the previous mainstream robot task, using Alexa’s services was close to being futile - “[Alexa] didn’t really do very much [...] I can’t tell it, say, hey Roomba, vacuum the bedroom, you know, because of course, I cannot set [the mapping feature] up. So for me, it’s kind of dumb to use Alexa because it really doesn’t do very much”. Hence, Jen resorted to using her smartphone application with the robot, which provided status alerts including the robot's power status.
    
    While limited functions are supported by some versions of the smart speakers compared to the phone application, two (Edward and Reena) participants preferred using a smart speaker with their robots since it is more efficient and supports hands-free interaction with the robot. As Edward mentioned, “I overall prefer to use Alexa. Once it was set up, I found it to be faster than pulling out my phone and going into the app and looking for the button that I wanted.” To add to the benefits of using the hands-free smart speakers with the robot, Reena said - “I really like to use Alexa better [than smartphone application], because then I don't have to figure out where my phone is, sometimes I keep losing it.”
    
    One participant, Sara, could not benefit from the hands-free interaction since she could not get her smart speaker to connect with the robot via Bluetooth. As a result, she turned back to the use of the smartphone application to understand the robot’s status. Edward also reported that setting up the connection requires users to have technical knowledge, which many users may not have. To avoid the trouble of externally setting up smart speakers with robots, Edward suggested embedding a smart speaker on the robot - “I would like to see a lot of [the robot’s functions] not have to be reliant on Alexa, because it's just one more thing to have to set up and have to, you know, make sure it works, so it would really be nice if it was all self contained where you could just issue commands to the robot itself directly. And then, and then have it reply verbally.”


    \textit{\textbf{Tracking by visual information.}} Some low vision participants, who have residual vision, can visually locate robots by observing the visual information on and around the robots, such as the contrast between the robot and the background, the light indicators, and other visual notification provided by the robot or its controller. 

        \textit{Colour contrast.} Some low vision participants can see the robot if it has high contrast against its environment. As Ara mentioned in the case of the vacuum robot, “I'm able to see the light and dark color contrast, and luckily the vacuums weren't the same color as the floor.” Similarly, in the case of the delivery robot, Ara could locate it since the robot’s colour contrasted with its surroundings - “[...] because I could see, because it was like black and silver, so it was, it was contrasting with the, with the ground and the surroundings, I was able to sort of tell tell where it was.” However, when there is no high contrast between the robot and its environment, it is difficult for the low vision participants to find the robot: “I wouldn’t be able to see where [the vacuum robot] was because it’s not contrasting with the carpet, because the carpet is dark as well. So, I had to like fumble around and try to find it, hoping I didn't step on it” (Ara). 

        Since it is hard to dynamically adjust the robot's color based on its surroundings, participants suggested that the robot’s appearance itself should present a high contrast to be more visible. As Ara suggested for the vacuum robot, “If it were like a black vacuum, it could have like a white ring on the outside, or, you know, vice versa. So at least the thing has some contrast, and I'd be able to see it.”

        \textit{Information on robot/remote controlled device display.} Some modern robots have a display, either on the robot itself or on a remote controller, to show its information to the users, such as the power status. Some low vision participants can read the information with their residual vision and some vision enhancement tools. “[The vacuum robot’s remote controlled device] has a very large display on top that has a dark background with the light letters. I can actually read those if I magnify them with my iPad” (John). 
            
        Unfortunately, for participants who are completely blind, the display feature was not accessible at all. Sara, who is totally blind, spoke about the inaccessibility of the display on the vacuum robot: “There's a display screen [on the vacuum robot] and I [am supposed to use] to go into the menus, but they are not accessible [because I'm totally blind].”

     
        \textit{Light indicators.} Eight participants reported the presence of indicator lights on the robot, which would either blink or light up in different colours to indicate the status of the robot. Some low vision participants can use the light to locate the robot especially when the noise generated by the robot is dampened by other sound in the environment. This was especially true in the case of the vacuum robot, as Ara mentioned, "Like my fridge is going on and off, you know that can impede on the sound [of the vacuum robot], so then I have the light [to locate the robot]". 

        However, the light is not visible to all low vision participants due to its small size and low luminance. John described the existence of this problem on his vacuum robot, “There's an [light] indicator for how full the bin is, which is totally useless for me because I can't detect it. It's a tiny, tiny, little indicator.” Even for the low vision participants who can see the light indicators, it is difficult to understand the meaning of the lights. For example, while Ara's vision is good enough to see the lights, she is color-blind and thus cannot distinguish the color to figure out the implication of the lights. 
         
        While some low vision participants can benefit from the light, it is completely inaccessible to people who are blind. For example, Jen described that the vacuum robot reset light was the only way to indicate whether the reset of the robot was successful. However, she cannot see the light, which makes it difficult for her to configure the robot. Instead of relying on visual cues, Jen emphasized the importance of having audible alternatives for the status alerts, "Because, you know, if you're blind, you're not going to be able to see the lights and know what's going on, so I think it's important for [the robots] to be as verbal and as interactive as possible." Even in the case of drones, Meg mentioned that the drone’s charging status is shown using an indicator light, which she could not see since she was totally blind.

        
        \textit{Camera on drones.} Some participants (Rita, Ahmed and Samuel) mentioned the presence of a camera on their drones. While it can stream its surroundings back to the user to help the participants track the drone, this feature is inaccessible to people with visual impairments. Instead, they could only estimate the drone's location based on the noise made by its propeller. As Rita said, "My husband and I are both totally blind. So you know, there is no audible output at all, so the camera was useless to us. The only way we knew where the drone was is because obviously it made a whirring sound."

    \textit{\textbf{Tracking by haptic feedback.}} Apart from using audio and visual cues, one participant, John, uses haptic feedback to track the vacuum robot’s status. His robot comes with a specialized remote controller (i.e., the FullCommand Remote for bObSweep PetHair Plus). When the robot gets stuck, the controller vibrates continuously to alert him. In general, John preferred haptic feedback the most compared to audio and visual feedback since it is a more universally accessible feedback that can be perceived by everyone, including people with multiple types of disabilities like hearing and visual disabilities. As he indicated, "For somebody like me [who is legally blind and deaf], the auditory and visual stuff, either is not useful or, you know, it might actually even be painful for me, but having the sense of touch is a universal identifier that everybody can associate with."
    
    \textit{\textbf{Delivery robot service provider dependent location tracking.}} In the case of delivery robots, once the food delivery order is placed, the first task is to locate the robot. Depending on the service provider, these robots provide different ways to locate the robot. John received text messages to notify him of the delivery arrival, while Ara had to use a website to track the robot location. However, the website relies on GPS and cannot locate the robot accurately in the last few meters. While sighted people can visually locate a nearby delivery robot, this last-few-meters way-finding problem is challenging for our participants with visual impairments\cite{saha2019closing}. Ara mentioned that she had to physically search for the robot when it arrived:
    
    \emph{“So I would check on the computer, because we have like a portal that you can log into to see where the robot was and where your food was, [but] it wasn't very specific. It was like, you know, say, your food is approaching your building. That's great, but when this building has several entrances, where's this thing going to meet me? So, I ended up like going outside of the building, walking around,and waiting for this thing to show up.”}

\textbf{(3) Other tasks}

    \textit{\textbf{Tasks unique to delivery robots.}} 
    
        \textit{Authentication of delivery.} A task that was observed only for delivery robots was authenticating the delivery service. John and Ara had different authentication experiences after locating the delivery robot. John authenticated the delivery robot using text messages - “You had to send a text message to let it know when you were ready [...].”

        On the other hand, Ara reported that there was not aware if there was any authentication required to pick up her delivery. She expressed her security concerns: "This [delivery robot service] didn't have any delivery authentication. This thing [delivery robot] just showed up, and you would hope that it was your food.” She suggested that the delivery robot should incorporate more secure authentication mechanisms to ensure that the right person received the delivery. Further, John, who had to use text messages to authenticate his delivery, emphasized on the need for a more secure approach, such as multi-factor authentication.
        
        \textit{Picking up the delivery.} Picking up the delivery from the robot is another task unique to delivery robots. Both John and Ara faced challenges when performing this task. Ara found it difficult to locate the food compartment on the robot, and she had to feel around the whole robot to find it. Since she has residual vision, she suggested adding some visual guidance to help her identify the food compartment, such as an arrow shaped light pointing to the food compartment. Meanwhile, John needed to press a button on the robot to open the food compartment to pick up the delivery. While he could locate the button because its color (red) contrasted with the colour of the robot (black), he emphasized that a person without color perception could find it difficult to locate the button since it was "only half the size of his palm" and was "more or less flushed with the rest of the device". 

    \textit{\textbf{Task unique to drones. }} 
    
        \textit{Obstacle Avoidance.} In addition to simply controlling the drone's moving direction, another important task is ensuring that the drone does not crash into obstacles. However, achieving this task is particularly difficult for people with visual impairments since they cannot visually detect obstacles in the path of the drone. For example, Samuel mentioned that his drone crashes many times because he cannot visually detect obstacles. 

        Reena thus suggested providing audio description about the drone's surroundings via its camera or having an autopilot option for autonomous navigation - “It would either need to be able to tell me accessibly what it sees so I could fly it or it would have to have some sort of autopilot”. Rita also suggested sending the camera's video stream to human service to get audio guidance. As she suggested, 
        
        \textit{“I think the only other option we would have to make the drone accessible would be to connect your camera with some [human] assistance that would be able to give you verbal feedback…just to know where it is, the beeping [when approaching an obstacle] is enough but to get more details, then speech would be great. Or even if you had the option to talk directly to it and say, where are you, or what's your problem, and get some verbal feedback”}
%% %% %% %% %%





%% %% %% %% %%
\subsection{Safety Around Robots}

Besides the accessibility issues when directly using the service robots, participants emphasize the safety concerns around mobile service robots as direct users and as bystanders. While all three types of robots have posed safety risks to our visually impaired participants, participants perceived drones to be the most dangerous type of robot. Figure \ref{fig:safety} shows participants' mean perceived safety scores for the different types of robots (perceived safety of vacuum robot: $mean = 6.00, SD = 0.89$; delivery robot: $mean = 5.50, SD = 2.34$; drone: $mean = 4.30, SD = 2.11$). The six participants who had experiences with vacuum robots and delivery robots reported a lesser average perceived safety rating for delivery robots compared to vacuum robots (perceived safety of vacuum robot: $mean = 5.67, SD = 1.03$; delivery robot: $mean = 5.5, SD = 2.34$), and the 12 participants who had experiences with vacuum robots and drones reported a lower average perceived safety rating for drones (perceived safety of vacuum robot: $mean = 6.2, SD = 0.78$; drones: $mean = 4.3, SD = 2.11$). John was the only participant who had experiences with all the three robots and he reported that drones are the most unsafe type of mainstream robots in general and interestingly, delivery robots are slightly safer compared to vacuum robots (perceived safety of vacuum robot: 6 ; delivery robot: 7, drones: 4) . In the following paragraphs, we intricately highlight participants’ safety perceptions around the different mainstream robots from both direct users' and bystanders' perspectives. 

\begin{figure}[h]
  \centering
  \includegraphics[width=0.75\linewidth]{Sections/safety.png}
  \caption{Average Safety Ratings (Scale: 1-7) for the Mainstream Robots. Note that the number of participants for each robot type is not the same.}
  \label{fig:safety}
\end{figure}

\textbf{\textit{Safety concerns as direct users.}} Fifteen out of the seventeen participants consider the low-lying vacuum robot as a potential tripping hazard when it is in the middle of the room. Eight participants even expressed fear of tripping over their vacuum robots, especially when the robot runs out of power and stops (or gets stuck) at some places before getting back to the charging dock. Although no participant tripped over the robot, two participants (Tim and Meg) accidentally kicked the robot a few times, and one (Jen) almost tripped over it. Jen described her "near-tripping" experience:

\emph{"There are times when I don't know where [the robot] is and I think I can trip over it. There was one time when [the dead vacuum robot] was just kind of in the middle of the floor and, I almost tripped over it, but I caught myself in time.”}

Moreover, Samuel, who had tunnel vision, expressed his frustration of visually watching out for the robot to avoid tripping: “Because I have low vision... one of my biggest headaches is tripping over things unless I'm looking down. I have to be looking down specifically and around the house [to avoid tripping over the vacuum robot].” 

To avoid tripping hazards caused by low-lying mobile robots, such as vacuum robots, Ahmed proposed to receive an audio feedback from the robot when in close proximity with it - "[Indicating that] you're too close to me or something like that, [vacuum robot can] play a sound or message if [vacuum robot] senses a human." However, if the robot's power is completely exhausted, it cannot provide any audio feedback to the user. 

Interestingly, the only safety concern expressed by one participant (John) with respect to delivery robots was the inability of the robot to navigate stairs. Besides locating the robots, physically reaching the delivery robots can also be difficult. John raised his concern that the delivery robot cannot climb stairs, so he had to go outside his apartment building to find the robot. He emphasized this concern by explaining how navigating stairs can be difficult and unsafe for people with visual impairments: “Stairs and blindness don't mix very well. So, it'll be nice if [the delivery robots] could get around the whole stair issue like the ability to deliver it in the apartment and not outside the building.”

In contrast to delivery robots, all the six participants (Nina, Meg, Reena, etc.) described various levels of fear about getting hit by the drone during use. As Meg mentioned, “There was a lot of several close calls of [the drone] attacking me as I didn't move [away from the drone] faster [because I could not hear the drone clearly].”  However, Sara, who used her grandchildren's toy drone very briefly, mentioned that she was not scared of flying the drone since she believed that drones mostly fly at elevated heights beyond human contact, “If [the drone is] coming close to my head, I need to duck, but usually, you know, they are way up there, so yeah, I don't have to worry about [getting hit by it].” Additionally, one participant, Reena, only felt safe when she flew the drone outside her house - “Outside [the house], I felt safe enough, but inside [the house], I didn't feel safe because it kept on crashing into the ceiling.” 

As a pacifier to the apprehension of getting hit by a flying drone, all the six participants who used drones suggested receiving more audio feedback from the drone, so that its location can be accurately perceived. As Meg described - "[...] adding like the option for some additional auditory component, so that you knew where [the drone] was the whole time [while flying]." 

\textbf{\textit{Safety concerns as bystanders.}} Besides direct user experiences, encountering mobile robots as bystanders can also raise safety concerns. We focus on participants' bystander experiences with delivery robots and drones since participants rarely have bystander experience with the domestic vacuum robots. 

Participants felt confused and anxious when they ran into a delivery robot on the sidewalk. They perceive the robot as an unfamiliar moving obstacle that has unclear intent and can potentially trip them. Thomas described his first encounter with a delivery robot:

\emph{"I encountered a robotic delivery device on the sidewalk in downtown San Francisco, and I was confused by it. And I think it was confused by me. I heard something on the sidewalk between loud traffic noises. And then, my cane detected [the delivery robot] and it was moving. And I think it stopped because my cane touched it. I reached out to see what my cane had touched that had been moving. And there was a box about the size of the shoe stand polishing box so it was probably 15 inches high by about 12 inches wide and 18 inches long, and I don't know what it was because I was by myself, but it moved. And I realized it was a box and it was probably a delivery box and when I got away from it, it started moving again and went on down the street. I was anxious about having heard it, having touched it with my cane and having it available to trip me."}

Further, Ara did not feel comfortable sharing the sidewalk with delivery robots since they take over the limited navigation space that is already challenging for people with visual impairments to use, which agrees with the findings of Bennett et al.'s work \cite{bennett2021accessibility}. As Ara said, 

\textit{“The sidewalks are narrow and really don't have enough space to have a robot running around with other pedestrians and then you have yourself and people who have a guide dog, cane or whatever it may be, trying to navigate the sidewalk plus listening to these, you know, ambient sounds around you... so yeah, there's definitely a lot of hazards that come with [the delivery robot].”}

Interestingly, instead of worrying about the robot hurting themselves, some participants were concerned about their white cane getting broken by the delivery robot. As described by Ara, “I really didn't have any trepidation about [the delivery robot] hurting me physically or injuring me, but I definitely had concerns that it would definitely break my mobility [cane] and then I would have a bigger problem.”

In order to avoid accidentally bumping into delivery robots on sidewalks, participants suggested various measures including increasing the height of the robot, alerting the robot's presence using unique audio signals, and using indicator flags on the robot. These measures could help bystanders, particularly PVI, identify the presence of the robot on sidewalks and take necessary precautions, such as moving away from the robot. To supplement these measures of alerting PVI about the robot's presence, especially for people who encounter the robot for the first time, Thomas suggested that the robot should be able to identify people with disabilities on sidewalks and give them space to pass the sidewalk safely - “I want Waymo and other autonomous vehicles [to] create entities [recognition systems] to identify mobility impaired people, old people, blind people, people in wheelchairs, and dog handlers [since] we may not completely interpret accurately the location of the the device [delivery robot], or how it is intended to interact with us.” Thomas’s quote draws a parallel with Salvini et al. \cite{salvini2021safety} statement on sighted bystanders’ lack of knowledge on public service robots. 

Compared to delivery robots, participants expressed more safety concerns towards drones. Since it is an object flying at heights above humans, participants felt scared that the drone could fall and hit them when losing signal or power. Meg mentioned that since these drones could be flying at higher speeds, the reaction time to these incidents would be minimal. The situation could be more dangerous for people with visual impairments because they cannot see the drone to determine the necessary action to avoid danger. John elaborated on the potential danger of a drone: “You know, a blind person is not going to know when they need to put up their hands on their face defensively...if you don't know what it is like, you don't even know if it has any sharp thing or something on it, and you don't know whether it's propellers are moving, its propellers could cut me.” 

To evade any potential danger caused by drones, John commented that there should be a law that restricts drone controllers to people who have completed the specific training to fly these robots in a safe manner, ensuring that the drone does not hurt any bystanders. Apart from safety policy implementation for drone flyers, Reena described adding safe landing features to the drone itself to reduce the impact of a crash - "[adding] some sort of backup system or something if [the drone is] going to be on the street, or like a parachute or something, or maybe the material it's made out of, so if [drone] slams into you, you won't get like seriously hurt." Further, as a bystander, Nina expressed that she would feel safe if there was a smartphone application that warned her about the presence and purpose of the flying drone - "I want to have like some kind of an app on my phone that would announce [if] there are drones near your location, and what they're trying to do." 
%% %% %% %% %%





%% %% %% %% %%
\subsection{Privacy Concerns Around Robots}

Participants also expressed privacy concerns around the robots. Similar to the perceptions of sighted people \cite{butt2021deployment}, \cite{LINTAN2021101462}, \cite{vcaic2018service}, the primary fear related to the violation of privacy is associated with the fact that robots, being smart devices, may have the capability to capture unsolicited information of users, such as personal videos, images, etc.  Having visual impairments aggravates this apprehension since it hinders such people from clearly recognizing the robot and its features. 

As a direct robot user, only John expressed concern for privacy with the use of robots. He described his concerns on the unauthorized access to private data that smart devices with speakers and microphones can have: “Some people don't like using things like Alexa, because they, you know, are worried about their privacy, because of the devices having cloud access to data across the network that somebody else could be accessing and it's especially distressing if you're blind, that, you know, somebody else is watching you when you can't be watching them. A lot of times speakers make people uncomfortable because, you know, well, they have a microphone and, you know, it's listening to me, and stuff like that…”. John’s fear of using smart speakers with robots follows the observations made by researchers on privacy concerns related to sighted people’s use of smart speakers \cite{lau2018alexa}, \cite{abdi2019more}, \cite{schonherr2020unacceptable}. 

On the other hand, six participants mentioned that their privacy could be violated as bystanders of robots, especially in the case of drones, since these robots have the ability to trespass their private property and take pictures. They felt the drone "invasive and threatening" (Thomas). Samuel described his anxiety about being around drones: “There is an invasive quality, because it probably has a camera... It's almost like these people are watching us with their drones.” Moreover, the privacy risk could be more severe to people with visual impairments since they lack the ability to visually detect the drone and determine whether they are being captured. As Thomas said:

\emph{“I don't want it coming over and inspecting me or hovering above my head...Also, where and why are big, big issues for me. Why is this thing here? What's it looking at? Am I involved? Is this observing me?”}
%% %% %% %% %%





%% %% %% %% %%
\subsection{Sighted Assistance to Support Interactions with Robots}

To overcome the accessibility and safety issues posed by the robots, participants seek help from sighted people, including both acquaintances and remote agents. Twelve participants mentioned using direct human assistance when interacting with or encountering robots.

\textbf{\textit{Help from sighted companions.}} Similar to prior research \cite{gadiraju2021fascinating}, \cite{bonani2018my}, eight participants (e.g., Thomas, Rita, Kat, etc.) asked their friends and family members to assist them when interacting with the robots. For example, when using vacuum robots, participants asked their friends and family to help start the vacuum robot (Rose and Rita), connect the robot to the robot application via WiFi or Bluetooth (Nancy), identify the button functionalities (Kat and Rita), check the cleanliness of the floor after the vacuum robot finishes cleaning (Thomas and Edward), find the stuck vacuum robot (Meg, Edward, and Nina), and do the maintenance of the robot (Rose).

Moreover, when encountering robots on the street, participants sometimes rely on their sighted companions to help identify and avoid the robots. For example, Kat asked one of the sighted people around to tell her what the moving object was. Participants also felt safer with their sighted companions when encountering a robot. For example, Thomas felt less anxious when he was with his sighted friend compared to encountering the drone alone. As he indicated, “Fortunately, I was with my sighted walking partner, so I didn't get anxious about it, but if I was out here by myself I would be really worried because it sounds like it's close.” 

\textbf{\textit{Remote Agents.}} Seven participants used remote agent service via smartphone or smartglass applications (e.g., Be My Eyes \cite{bemyeyes} and Aira \cite{aira}) to conduct visual tasks, such as locating a stuck vacuum robot, and recognizing the non-tactile buttons on the robot. For example, Tim described his use of the mobile application, "Be My Eyes'': “I use [Be My Eyes] like if I go to the usual spots where [the vacuum robot] is not there and I don't feel like crawling around on my hands and knees or whatever.”

\textbf{\textit{Customer Service.}} To use his vacuum robot, Tim always seeks help from the customer service. However, the instructions provided by a sighted agent are not helpful for him - The sighted agent uses only visual cues (e.g., colors of the robot components) as references during communication rather than tactile cues, which is not accessible to people with visual impairments. Tim described his experience where the customer service was giving him instructions to replace the brushes for his vacuum robots:
    
\emph{“There was a little bit of issues where they just couldn't communicate with me because, you know, they're sighted and I'm blind and the landmarks that they are using and trying to describe aren’t useful to me. So, you know, trying to get them to describe something to me in the language that I could understand, what I'm feeling versus what they're seeing...was a little bit of a challenge. For example, when you're going to replace the brushes underneath the [vacuum] robot. There's this tiny little lever that you have to squeeze this little trigger kind of thing in order to be able to open [the robot] and get the brushes. I couldn't get them to describe that tiny little lever because it's so small that if you don't know exactly what you're feeling for and where it is... It's pretty invisible, so I needed them to be able to say, okay, the lever that you're looking for is right next to this particular wheel right, next to this landmark or whatever, but they just kept saying, Oh, it's the blue lever... That doesn't do me any good. I need you to tell me, you know, is it near the left wheel or the right wheel, and depending on which way the robot is facing, you know, which way is left and which way is right.”}

Moreover, Tim expressed his disappointment about the customer service would not take his suggestions on improving the accessibility of the robot because of copyright infringement: 

\emph{“There's a large, large component of the technology built into this that I can't use. And the fact that, you know, when I call them and say hey, here's the problem that I have and here's, you know, as a blind person, a couple of easy solutions that I think would fix it, and they won't, and they refuse to listen to me, claiming that it could be a patent infringement if I give them an idea, and they run with it and build it into the robot, they're claiming I could turn around and sue them for copyright infringement.”}
%% %% %% %% %%





%% %% %% %% %%
\subsection{Extended Applications of Mainstream Robots}
Excluding PVI's experiences on the three mainstream robots discussed in this study, participants also revealed potential applications of mainstream robots including autonomous driving cab service, package pick-up service, and drones for monitoring children in parks. Thomas described the package pick-up service by robots - “I guess I would have to say, UPS Store send me a bot [to] pick up the box. I guess its operation would be guided by the app on the phone. [...] This is important as an ultimate use of bots if they're going to be ubiquitous.” Further, he explained how he expected autonomous driving cabs to interact with PVI - “I was thinking about, if there was an autonomous vehicle that came to pick me up, it needs to identify me, because I don't know one vehicle from another stopping in my street, or on the street. It would have to be able to identify me, notify me that of its proximity and how to find it.” In addition to delivery robots and autonomous driving vehicles, Rita envisioned having drones to keep an eye on her child in the park - “I could use a drone to position it above, let's say, a soccer field, where my child is playing soccer. And the drone would be able to track my child and maybe give feedback, you know, even in a crowded place [like] an amusement park, you know, that would be helpful.” All these various insights clearly indicate that PVI are interested in the development of mainstream service robots, and could benefit in different ways from their use. 
%% %% %% %% %%



==> Related Work/Copy.tex <==
\section{Related Work}

\subsection{Sighted People's Experiences and Perceptions of Mobile Service Robots}

Service robots perform challenging and repetitive tasks for humans \cite{ServiceRobotDef}. Such robots range from partial autonomy that involves human-robot interaction to full autonomy without active human intervention. Service robots can be classified into two major categories according to its use and operators---personal service robots and professional service robots \cite{zielinska2016professional}. Personal service robots are used for non-commercial tasks by lay persons, such as domestic vacuum robots, remote presence robots, and automated wheelchairs, while professional service robots are usually operated by properly trained experts for commercial tasks, such as delivery robots and surgery robots. 


A wealth of prior research has explored people’s experiences and attitudes when interacting with different service robots \cite{young2009toward,schneiders2021domestic, dautenhahn2005robot}, such as domestic vacuum robots \cite{forlizzi2006service, de2019would, sung2007my}, delivery robots \cite{jennings2019study, lee2020robots, pani2020evaluating}, and drones \cite{culver2014battlefield, eissfeldt2020acceptance,lidynia2017droning}. For example, Forlizzi and Disalvo \cite{forlizzi2006service} conducted ethnographic studies with 14 families to explore the effect of a Roomba vacuum robot on home ecology. They found that the adoption of Roomba changed people's cleaning practices by enabling multitasking and planned cleaning, as well as influencing the roles of family members in housekeeping by engaging men and children in cleaning. Delivery robot is an emergent shared robot that has recently attracted HCI researchers' attention, especially during the COVID-19 pandemic. Via a survey with 473 participants, Pani et al. \cite{pani2020evaluating} explored the consumers’ preferences, trust, and attitudes towards the deployment of autonomous delivery robots during the pandemic. The study showed an overall positive attitude towards the delivery robots with 61.28\% customers indicating willingness to pay for the robot service. Moreover, Lee and Toombs \cite{lee2020robots} explored the public perceptions of Starship delivery robots by analyzing Reddit posts, finding that people perceived the robots differently as mascots, friends, or aggressive gangs, and expressed affections for the robots.


% drone use - focus on experiences of sighted people with drone applications like videography
%Human drone interaction  - https://hal-enac.archives-ouvertes.fr/hal-03299076/document
%Drone is another type of mainstream robots that are being used for a variety of applications, including videography \cite{kang2018flycam}, delivery \cite{huang2020new, manna2021route, ursulian2021last}, and navigation \cite{brock2018flymap}. With the burgeoning use of drones, there has been an abundance of research on Human-Drone Interaction (HDI) exploring and determining the best way for humans to interact with drones. For example, Cauchard et al. \cite{cauchard2015drone} conducted a Wizard-of-Oz study with 19 participants, where each participant was asked to perform a set of tasks, such as making the drone click a selfie, stopping the drone, etc. One researcher controlled the drone according to the actions of the participants while the participants performed the tasks. It was found that people like to interact with drones in ways similar to how they would interact with other people or a pet. With these observations, the researchers came up with design recommendations for a "multimodal interaction" that includes gestures and voice commands to control drones. In another HDI study, Obaid et al. \cite{obaid2020domestic} explored the applications of drones in domestic spaces by studying 61 relevant papers. They found that navigation was the most prominent drone application, which primarily included guide drones for tourists and people with visual disabilities.


%%  \begin{figure}[!htb]
%%    \centering
%%    \begin{subfigure}[b]{0.30\textwidth} 
%%      \includegraphics[width=\linewidth]{Sections/vacuum robot.jpg}
%%      \caption{}
%%      \label{subfig-1:dummy}
%%    \end{subfigure}\\[2ex]
%%    \begin{subfigure}[b]{0.45\textwidth}
%%      \includegraphics[width=\linewidth]{Sections/delivery_robot.jpeg}
%%      \caption{}
%%      \label{subfig-2:dummy}
%%    \end{subfigure}
%%    \hfill
%%    \begin{subfigure}[b]{0.38\textwidth}
%%      \includegraphics[width=\linewidth]{Sections/drone.png}
%%      \caption{}
%%      \label{subfig-3:dummy}
%%end{subfigure}
%%    \caption{Examples of the the three mainstream robots: a) Remote controlled vacuum robot \cite{vacuum}; b)Picking up food delivery from delivery robot \cite{d'antino_2020}; c) Remote controlled drone with display \cite{jessica}}
%%    \label{fig:dummy}
%%  \end{figure}

%\begin{figure}[h]
%  \centering
%  \includegraphics[width=0.75\linewidth]{Sections/combined_robots.png}
%  \caption{Examples of the the three mainstream robots: a) Remote controlled vacuum robot \cite{vacuum}; b)Picking up food delivery from delivery robot \cite{d'antino_2020}; c) Remote controlled drone with display \cite{jessica}}
%  \label{fig:robots}
%\end{figure}

Besides the direct interaction with robots as users, researchers have also explored people's experiences and attitudes when they come across publicly used service robots as bystanders, revealing their concerns around the robots. %While there are a multitude of factors that serve as proponents for bringing robots into public spaces, such as the development of environment friendly delivery facilities \cite{schaudt2018delivery}, the public use of robots gives rise to apprehensions about the safety and privacy of people using these spaces.  
%Researchers have pointed out that people's safety concern with having robots in public spaces is associated with the fact that they may not be fully aware of the robot's behaviour, capabilities, and purpose of existence. 
For example, Salvini et al. \cite{salvini2021safety} pointed out that pedestrians and bystanders faced both physical and psychological safety hazards in the presence of mobile robots in public spaces since they lack awareness on how to interact with the robots and the clarity of robots' intentions. They highlighted the needs for standards and guidelines for public-use robots that protect bystanders' safety and rights. Thomasen \cite{thomasen2020robots} also argued that civilians' space and comfort must be prioritized over robots' use of public space.
In addition to safety concerns, researchers have also analyzed the potential privacy risks posed by the publicly used robots \cite{butt2021deployment, LINTAN2021101462}. For example, Tan et al. \cite{LINTAN2021101462} studied 1050 Singaporean residents' responses to a questionnaire, asking about their experiences of encountering flying drones in public space. They found that people's primary fears and concerns were the loss of privacy and unauthorized filming by the drones. 

While prior research has thoroughly investigated people's robot experiences and concerns from both user's and bystander's perspectives, this research has mainly focused on people who are sighted. Unlike sighted people, PVI can face additional accessibility challenges and more severe safety and privacy risks when using and encountering mobile service robots. However, their unique challenges and needs remain understudied. 


%it is clear from the abundance of existing research that mainstream robots in public spaces harbour safety and privacy issues for sighted civilians, these concerns are not thoroughly explored for PVI. In fact, these concerns could pose elevated hazards for PVI since they may not have the ability to perceive the presence of the robots unlike sighted people.

%Butt et. al \cite{butt2021deployment} examined drones with artificial intelligence and found a great threat of unsolicited imagery and videography posed by these drones to people in public spaces. In a similar context,


%Therefore, with most of the research focusing on the experiences of sighted people with mainstream robots, there is limited research on the accessibility, safety, and privacy concerns associated with mainstream robots for PVI. 

\subsection{Specialized Assistive Service Robots for People with Visual Impairments}

Robotics research for PVI has mainly focused on designing and building specialized assistive robots to facilitate various daily tasks. Most assistive robots have been designed to enable PVI to navigate surrounding environments \cite{guerreiro2019cabot, kulyukin2005robocart, tachi1984guide, kulyukin2006robot}. For example, Guerreiro et al. built CaBot \cite{guerreiro2019cabot}, a suitcase shaped robot that can guide blind people via vibro-tactile feedback to help them avoid obstacles on the path and arrive a destination safely. They evaluated CaBot with ten blind participants who performed navigation tasks, finding that users felt comfortable, safe, and confident when navigating with CaBot. Some guide robots were designed for specific scenarios, such as a grocery store. For example, RoboCart \cite{kulyukin2005robocart} was a robotic shopping assistant designed to help visually impaired people navigate a grocery store while carrying purchased items. Besides on-the-ground robots, researchers have also leveraged flying drones to guide visually impaired users during navigation \cite{avila2015dronenavigator, al2016exploring}. For example, Avila et al. \cite{avila2015dronenavigator} proposed a wearable bracelet prototype with a small drone mounted on it. When a blind user verbally assigned a navigation task to the drone, the drone started flying and guided the user to the destination. 

%Graether et al. \cite{graether2012joggobot} designed Joggobot, a robot that flies to accompany joggers. This study resulted in robot design insights for physical exertion activities. 

In addition to navigation, researchers have also designed robotics technologies to support other tasks. For example, Huppert et al. designed GuideCopter, a drone-based system to assist visually impaired people in an object localization task. With GuideCopter, a drone was tethered to a blind user's finger, thus providing fine-grained haptic feedback to guide the user's hand to a target object \cite{huppert2021guidecopter}. Moreover, Bonani et al. \cite{bonani2018my} explored the potential of a collaborative assistive robot that provided physical instructions and feedback to guide blind users' hands in an assembly task. In an evaluation with 12 visually impaired participants, they found that participants perceived the physical assistive robots to be warmer, more competent, and more useful than a voice-only assistant.  

While various specialized assistive robots have been designed to empower PVI, the mainstream service robots, which are more commonly used to support people in all kinds of environments and tasks, can still pose severe barriers to PVI, further marginalizing them as the robotics technology advances.  
%As such, it is critical to identify PVI's challenges and needs around different mainstream service robots, promoting equal access to this emerging technology. 

%The use of assistive technologies, whose design features conflict with the universal design standards, have resulted in increased visibility of people using these devices in public spaces. Consequently, this creates an apprehension for people with disabilities to freely incorporate these devices into their daily living. Specialized assistive technology may stigmatize people with disabilities, leading them to abandon the technology altogether \cite{parette2004assistive}. By improving the accessibility of the commonly used service robots, the adoption and acceptance of the mainstream robots by PVI can be enhanced, thus diminishing the stigmatization inherent with the creation of assistive robots. 

\subsection{People with Visual Impairments and Mainstream Robots}
%mainstream robot not accessible to PVI - https://www.mdpi.com/2079-9292/10/5/561
%While enhancing the adoption of mainstream robots by PVI can eradicate their feelings of being alienated from mainstream technology.
With the growing popularity of various service robots, some recent research has started exploring PVI's expectations and needs for the mainstream robots. From example, to enable building service robots to guide blind people properly, Azenkot et al.\cite{azenkot2016enabling} conducted participatory design sessions, where three designers and five visually impaired users collaboratively design the interaction and behaviors for a robot guide via brainstorming and discussion. The study specified design recommendations different PVI-robot interaction stages, such as how to initiate the contact with a visually impaired user, how to properly guide the user, and how to alert her of obstacles and turns. Instead of focusing on one specific type of robot, Bonani et al. \cite{bonani2018my} explored blind people's perceptions and visions on general service robots via a set of focus group discussions. They found that, while having concerns about robot control, reliability, and maintenance, participants expected that robots would be integrated in their daily life and assist with various tasks such as navigation, housekeeping, and social interactions. However, these studies focused on discussing the ideal service robots for visually impaired users without investigating their real-world experiences with robots. In fact, Bonani et al. has clarified that most participants had never interacted with a real robot. 

Moreover, Qbilate et al. \cite{qbilat2021proposal} proposed a set of accessibility design guidelines for human-robot interaction by adapting and extending existing accessibility standards and guidelines for other mainstream user interfaces (e.g., web sites, mobile applications). The guidelines were evaluated by seventeen human-robot interaction (HRI) designers from four aspects, including usability, social acceptance, user experience, and social impact. Most designers felt the guidelines helpful and were willing to use the guidelines in their future design. Nonetheless, no people with disabilities have been involved in the development and evaluation of the guidelines. 


%Mainstream robots pose multiple forms of accessibility barriers that prevent PVI from extracting the benefits of using these robots. Hence, it is crucial to identify and comprehend the concerns surrounding PVI's use of mainstream robots. Qbilat et al. \cite{electronics10050561} state that PVI may find it difficult to differentiate and recognize the hardware and software elements of the robot. Additionally, assistive technologies used by PVI (e.g., screen readers) may not be compatible with the robot's interface. Hence, considering all the types of disabilities, including auditory, visual, motor and cognitive disabilities, a set of HRI design guidelines were developed by the researchers and evaluated by 17 HRI designers with the help of Likert Scale and open-ended questions. However, not only is there no evidence provided to back the statements related to the PVI's accessibility issues with mainstream robots, but also the proposed accessibility guidelines do not take into account other forms of concerns, such as the inherent safety and privacy barriers associated with PVI's experiences with mainstream robots. 

%an exploratory study, in which most of the participants opined that the size of the robots must be directly correlated to the application of the robot. For example, navigation robots must have a small size in order to navigate efficiently in indoor/outdoor spaces. It was also expressed that not only should robots be available throughout the day to perform tasks efficiently and quickly, but it is also important for robot designers to incorporate the capability to avoid collisions with people by making its presence known. The participants of the study also professed that way-finding, housekeeping, educational provisions and social interactions were the most important use cases of robots. While these insights were purported to be beneficial for robot designers attempting to create one from scratch for visually impaired people, deductions on improvements that could be made on existing service robots to enhance accessibility were not presented. 

%provide design specifications for the commonly used Building Service Robots (BSRs) that could also be used to guide blind people to the various parts of large buildings, apart from performing various services to people in general. This study aimed at understanding the current navigation techniques used by blind people, and how BSRs could be leveraged as guides for blind people. A participatory Wizard-of-Oz study design involving one-on-one interviews, group discussions and individual design sessions with technical designers and PVIs lead to design insights related to human-robot contact initiation, convenient path navigation, obstacle avoidance, and human-robot contact termination. Although this research serves as a good example of developing design improvements on currently available robots to enhance its accessibility to visually impaired people, it focuses only on a particular type of mainstream robot.  

There has been little work exploring PVI's firsthand experiences and challenges around the mainstream service robots. Gadiraju et al. \cite{gadiraju2021fascinating} surveyed 59 visually impaired people and conducted interviews with 13 of them to understand their motivation and experiences with drone piloting. They found that PVI showed a general curiosity about the drones and flied drones for different reasons, such as engaging in family activities and collecting environment information. The study also highlighted participants' challenges and preferences on different drone control approaches, suggesting multiple control and feedback configurations should be supported based on users' environments and preferences. Moreover, Bennett et al. \cite{bennett2021accessibility} touched on the safety concerns of pedestrians with motor-related disabilities when encountering delivery robot on the sidewalk. Via interviews with activists with disabilities, government officials, and commercial representatives, they revealed the barriers created by the evolving micromobility technology (e.g., bikeshare) and related policies for people with disabilities. However, their work mainly focused on the policy and regulation perspective of micromobility technology instead of service robots. Only one participant who's a power wheelchair user shared her experience with delivery robot. There is thus a lack of knowledge in the accessibility field on how people with visual impairments negotiate the growing number of service robots in their daily life. 

Our research seeks to fill the gap in prior research by deeply investigating PVI's experiences and needs with different mainstream service robots, from both users' and bystanders' point of view, thus deriving design guidelines for more accessible and safe human-robot interaction. 

%Different categories of drone users were identified, including family flyer, environment explorer, navigator, aviation enthusiast, and technology fan. For example, one participant mentioned that observing a family of sighted members fly these drones to take nice pictures inspired them to try out drones to take pictures of their family (family flyer). In most cases, participants sought help from sighted friends and family members to control drones mainly because piloting drones forces the user to rely on visual information, which is inaccessible to PVI.

%While this study highlights interesting insights related to PVI's use of drones, it fails to provide PVI's experiences of mainstream robots in general.


%why do PVI use drones - https://hal-enac.archives-ouvertes.fr/hal-03299076/document 
% In addition to drones, Bennett et al. \cite{bennett2021accessibility} elucidate the accessibility and safety concerns engendered with the rising presence of "micromobility devices", including delivery robots, e-scooters, etc., on sidewalks. The researchers interviewed government officials, people with disabilities, disability activists, and mobility device representatives to find that these devices block the sidewalks for pedestrians posing safety hazards while crossing roads. These devices also block the wheelchair ramp for people with disabilities. However, this research focuses only on the PVI's mobility barriers in the presence of delivery robots in public, and ignores the potential safety hazards and accessibility barriers posed by other forms of mobile service robots, such as vacuum robots and drones. This research also misses out on PVI's interaction experiences during the direct use of mobile service robots. 






%To bridge the gaps of prior research, this study explores PVI's experiences, as both users and bystanders, with three popularly used mainstream service robots (vacuum robots, delivery robots, and drones), unearths the associated accessibility, safety and privacy issues, and proposes robot design guidelines to enhance PVI's experiences with mainstream mobile robots in general. 















==> Sections/6-Limitations_and_Future_Work.tex <==
\section{Limitations and Future Work}

Our study has some limitations. First, we focused on three types of mobile service robots (i.e., vacuum robots, delivery robots, and drones) used, and people's experiences with these robots to derive general robot design considerations. While our robot selection considered both popularity and coverage (e.g., personal vs. shared robots, low-lying vs. flying robots), there could be specific robot types that we have not covered, which could lead to new accessibility needs and design guidelines. In the future, we will expand our study to more diverse robot types, such as social robots and humanoid robots, to construct a more complete understanding on PVI's robot experiences. 

Second, the number of participants for each type of robots were not equally distributed in our study: all participants had experience with vacuum robots, while only partial participants used or encountered drones and delivery robots, which resulted in relatively limited data for the drones and delivery robots. This is not surprising given that the vacuum robot technology is more mature and widely used than drones and delivery robots. %Our initial survey (Figure \ref {fig:survey}) has confirmed this uneven distribution.
As service robots become more popular, we plan to recruit more participants for the emerging types of robots (e.g., delivery robots) to enrich our data. Moreover, we conducted a remote interview study because of the COVID-19 restrictions. In future, a contextual inquiry study observing PVI's interactions with service robots will be considered to enhance the data.

%this study was conducted with participants whose experiences with mainstream service robots were not uniformly distributed across the three mobile robots. This was because we recruited participants who had experiences with at least one of the three mobile service robots. While we considered the possibility of recruiting equal number of participants for each robot type, our survey responses (Figure \ref{fig:survey}) showed us that there are quite a few PVI who use delivery robots and drones compared to vacuum robots. This is because the vacuum robot is a relatively mature field of technology whereas delivery robots and drones are still emerging forms of robotic technology. In our future work, as service robots become more popularly used, we plan to recruit equal number of participants in each robot category.

 
